Tangle Centric Networking (TCN)

Today's Internet is heavily used for multimedia streaming from cloud backends, while the Internet of Things (IoT) reverses the traditional data flow, with high data volumes produced at the network edge. Information Centric Networking (ICN) advocates against a host-centric communication model which is promising for distributed edge computing environments and the execution of IoT applications in a decentralized fashion. By using naming schemes, data is tightly coupled to names instead of hosts which simplifies discovery and access to data and services. However, the tight coupling challenges network performance due to additional synchronization overhead of large data volumes and services. We present Tangle Centric Networking (TCN) -- a decentralized data structure for coordinated distributed applications and data exchange following principles of ICN. TCN can react on data and service changes and update them accordingly in network nodes, provide distributed data structures and enable cooperative work on the same data without huge overhead by using Tangles for coordination. We implemented TCN in simulations and evaluated the concept against a base line scenario.

==> Tangle Centric Networking/background.tex <==
\section{Background \& Related Work}
\label{sec:background}

As we move toward a distributed edge computing environment, computation-centric network architecture defines a need to support decentralized and distributed computations.
The following sections will present some background and related work. 

\subsection{Information Centric Networking}
\label{sec:background:icn}
ICN describes a paradigm which puts data as the first class citizen in the network by separating content from its physical location.
We refer the term ICN to the network principles introduced by Jacobson et al.~\cite{jacobson2009networking} including architectures such as Named Data Networking (NDN)~\cite{zhang2014named}. 
By changing the addressing scheme using content identifiers (e.g., hierarchical naming schemes), ICN achieves a loosely-coupled communication model directly on the network layer.
This is in stark contrast to host-centric deployments where devices need to connect to specific nodes using their IP address. 
Therefore, ICNs are promising for data transport in deployments at the network edge as well as in IoT environments as there is no need for the network to track the location of individual nodes~\cite{Amadeo:ICN:IoT:2016, grewe2017information}.

%\DENNIS{More information on manifests and delete MTU arguementation}

Content in ICN is represented by so-called \emph{Named Data Objects} (NDO) that have identifiers, but that are usually not associated to a single or specific physical node in the network.
To transfer large volumes of data in an ICN, NDOs are structured into smaller chunks to fit into the maximum transmission unit of the underlying network. 
ICNs provide several solutions to discover the identifiers of chunks of a particular NDO including Manifest (e.g., FLIC~\cite{tschudin2016file}) or DNS-like resolution system such as NDNS~\cite{afanasyev2017ndns}. 
For example, FLIC is build like a UNIX directory. From a root manifest (in UNIX terms: root-directory) it points to chunks (in unix terms: files) and to the next manifests (in UNIX terms: directories). Each manifest can contain further manifests or chunks. Thus, FLIC represents a tree, where manifests are inner nodes and chunks are trees. 
This is a very efficient data structure to find certain chunks, since the search time is reduces from linear to logarithmic.
However, to support the execution of distributed application on top of ICNs, any changes to data requires updates of the NDO descriptions to provide access to vital data. 
For example, FLIC Manifests often have to be re-created entirely every time a change to a NDO happens, since each of the manifests contains signatures of the chunks/other manifests it is pointing to.

Addressing this issue, distributed data synchronization protocols have been proposed in the literature to support multi-party communication in ICNs (cf.~\cite{Shang:NDNSync:2017}).
Examples include ChronoSync~\cite{Zhu:ChronoSync:2013}, VectorSync or PSync~\cite{Zhang:PSync:2017} featuring different design rationals in naming schemes, and state propagation. However, as we move towards edge computing environment, these solutions have not been evaluated in the context of compute-centric networking architectures.

%\subsection{Compute-Centric Architectures}
%\label{sec:background:ccn}

%Despite its conceptual fit to IoT deployments (e.g., Amadeo et al.~\cite{Amadeo:ICN:IoT:2016}, the vast majority of ICN approaches to date focus on distribution of static content. 
%Compute-centric architectures extend ICNs to execute functions/services at any element in the network such as intermediate/edge routers and end-user devices.
%Therefore, computations are location independent and the network will resolve the optimal location to compute a result.
%Examples of such architectures include NFN~\cite{sifalakis2014information}, NFaaS~\cite{krol2017nfaas}, or CFN~\cite{krol2019compute}.

%As in ICNs, compute-centric architectures use naming schemes to invoke functions/services or to provide access to computation results.
%In order to be able to resolve the (complex) computation requests, compute instructions are modeled as compute graph, evaluated by network elements using a naming scheme. 
%For example in NFN~\cite{sifalakis2014information}, the compute-graph is models as a set of $\lambda$-expressions directly encoded within a name, representing a set of stateless, invokable functions.
%While processing a compute request, NFN nodes evaluate and instantiate functions according to the naming structure of the compute expression.
%However, the encoding of a compute graph as part of the name presumes that it is known in advance.
%Similarly like NFN, NFaaS~\cite{krol2017nfaas} encodes certain function invocation aspects (e.g., time-constraints for efficient task scheduling) directly in the naming scheme.
%However, the framework focuses on stateless computations and does not provide mechanisms to realise stateful computations.

%CFN~\cite{krol2019compute} supports both stateless functions and stateful actors.
%It defines compute graphs as separated inputs modeled as conflict-free distributed data types (CRDTs)~\cite{Shapiro:CRDT:2011}. 
%The computing platform uses the graph for evaluation and performs flexible load management and performance optimizations by taking function/actor and data location into account.
%Based on the information within the CRDT, the execution of a computation can lead to arbitrary instantiation of new computations in the network in order to fulfill the computation request.

%\DENNIS{Final sentence to close the section missing - but what is a good one? CRDTs to hand over to next section?}

\subsection{Distributed Storage \& Ledger}
\label{sec:background:dlt}

In distributed systems, the CAP theorem (also called Brewer’s Theorem) poses that a system can have only two of three desirable properties: \emph{consistency}, \emph{availability}, and \emph{partition tolerance}~\cite{Gilbert:CAP:2002}.
However, trade-offs can be achieved by explicitly handling partition tolerance in order to optimize consistency.
%While in ICNs, as well as in compute-centric architectures, partition tolarance and availability are addressed via the loosely coupled communication model and replicating NDOs at forwarding nodes, consistency describes a challenge.
For example, CFN uses CRDTs to describe the compute graph the platform should execute~\cite{krol2019compute}.
However, CRDTs only guarantee \emph{eventual consistency} demanding for global consistency - the entire data structure has to be updated in case of changes~\cite{Shapiro:CRDT:2011}.
In recent years, distributed ledger describes a technological infrastructure representing consensus by allowing to access, validate and record data across multiple parties in a distributed fashion~\cite{swan2015blockchain}.
The Blockchain~\cite{swan2015blockchain} implements a distributed, append-only structure consisting of connected blocks. 
Examples based on the technology include Bitcoin~\cite{nakamoto2019bitcoin} or Ethereum~\cite{Ethereum}.
In the context of compute-centric architectures, the SPOC~\cite{krol2018spoc} approach uses Ethereum to record outsource computations, executed by 3rd party nodes in the infrastructure, able to validate changes.

Instead of recording entries as an append-only structure of connected blocks, the Tangle~\cite{popov2018tangle} technology, which is the data structure behind IOTA~\cite{IOTA:2021}, implements a directed acyclic graph (DAG) for storing transactions.
Every new transaction has to approve at least two previous transactions to be recorded in the Tangle. A tip is a not yet approved block. Thereby, the \emph{tips selection algorithm} chooses two tips that should been approved. The 
algorithm makes sure that tips are chosen in a way, that the tangle will reach convergence quickly.

Based on this concept, Tangles build their consensus development based on the number of accepted predecessors in the Tangle, while not relying on a proof-of-work concept (e.g., in Blockchain) or on a certain time interval (e.g., as in CRDTs).
Figure~\ref{fig:blockchain:tangle} illustrates the differences between the Blockchain and Tangle technology.
If status changes happen, nodes can still operate on old data as they are not immediately evicted from the Tangle structure, allowing for situations in which the result of the operation might be validated.

\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{Figures/blockchain_vs_tangle.pdf}
    \caption{Illustration of the characteristics of the distributed, append-only data structure of Blockchain and Tangles.}
    \label{fig:blockchain:tangle}

\end{figure}

==> Tangle Centric Networking/concept.tex <==
\section{Tangle Centric Networking Architecture}
\label{sec:tangles}

The tight coupling of content identifiers challenges the introduction, and thus, the discovery of newly generated content in ICNs and compute-centric approaches as well (cf. Section~\ref{sec:intro}).
In order to address this problem, we propose Tangle Centric Networking (TCN).

TCN enhances the design principles of Interest-based ICN architectures (e.g., NDN) with the Tangle technology~\cite{popov2018tangle} to improve data retrieval of content in ICNs (see Section~\ref{sec:background}).
%It is based on the pull based mechanism using Interest Messages and Named Data Objects (NDO).
Like in ICNs, TCN uses naming schemes to request for NDOs and supports Manifests to query the network for large objects.
Large objects are divided into chunks, while each chunk  is associated with a content identifier, managed in a Manifest (e.g., FLIC~\cite{tschudin2016file}).
%An interest message contains a name and is send into the network to receive a NDO with the same name. The core data structures are a Content Store (CS), a 
%Pending Interest Table (PIT) and a Forwarding Information Base (FIB). 
%However, there is one additional data structure the Manifest Synchronization Table (MST). 

%Each NDO in TCN is split into chunk of roughly the same size. All chunks of a NDO are listed in a manifest. A manifest is represented by a tangle. 
%A Tangle is identified by a network-name, so that it can be requested as manifest for fetching data objects.
%According to the handling of NDOs in ICN, large objects are divided into chunks.
%Each chunk is assigned with a content identifier, listed in a Manifest (e.g., according to FLIC~\cite{tschudin2016file}).

In TCN, the Manifest of each NDO is represented as a Tangle, associated with a content identifier that can be requested within an ICN.
Each Tangle represents a set of chunks of a NDO (or the entire NDO) in a structured way.
In case a change happens to a NDO, and therefore, to a set of chunks of the NDO, the characteristics of a Tangle allows network participants to acknowledge to the latest status of it and thus, to achieve consensus.
As a result, Tangles in TCN represent a common structure handling all versions of a particular NDO. 
It allows a consumer to selectively request for different versions of a NDO, without resolving several identifiers for each Manifest as required in FLIC.
Furthermore, the special update and synchronization characteristics of Tangles simplify the handling of changes of NDOs and is promising to improve the performance of updating Manifest.

\subsection{The Design of Tangles in TCN}
\label{sec:tangle:design}
A Tangle in TCN is represented by two elements: A \textbf{core element} -- representing a part of a NDO Manifest, containing a list of names of associated chunks, and an \textbf{acknowledgement element} -- representing a meta-information block to assist consensus. 

The \emph{core element} stores the name as well as the hash of each associated chuck, used by nodes to query the network for data.
Each Tangle is signed by the producing node using digital signatures to ensure data integrity and authenticating the originator of the Tangle. 
In order to point to the next subsequent core element of the Tangle which contains the information to the next chunks, the element maintains the hash value of the previous core element and the hash value of at least one further chunk to form the initial Tangle. 
As a result, the Tangle created is represented as a DAG of elements (see Figure~\ref{fig:CoreElementTangle}).
The verification degree of a core element is the number of incoming edges of acknowledgements, while a Tangle \emph{tip} describes an element with no incoming edges.
By referring to the \emph{precedent} chunks instead of following ones (e.g., as designed in BlockChain~\cite{swan2015blockchain}), a data flow driven processing of Tangles is ensured by design.
Chunks within a Tangle are already available in the network to be requested by consuming nodes, while subsequent chunks are not yet created.

%The task of a core element is to store the name and the hash of a chunk, so a node can identify the data to be requested from the network. To form a chain, a core element contains the hash value of the previous core element, pointing on the previous chunk and the hash value of at least one further chunk to form the initial tangle. Only the first chunk does not point on any other chunk and the second chunk only points on the first chunk. By pointing only on precedent chunks and not on following chunks, we can ensure that the manifest structure is ready for streaming, where chunks are already fetched while other chunks are not yet created. Each chunk itself as well as each element in the Tangle is signed by the private key of the producer.

As core elements of a Tangle might get created and appended to the overall Tangle structure in irregular time intervals, a mechanism to model consensus is required. 
To model it, an acknowledgement element describes a meta-information block associated with each core element (see Figure~\ref{fig:CoreElementTangle}). 
Every time a core element is synchronized and accepted by another node in the network, an acknowledgement element for the particular core element is appended by the synchronizing node.
This way, a single node can only append one acknowledgement per appended block. Thus, with the knowledge how many nodes are synchronizing, a node knows when a consensus was established for a block. 
In TCN, we do not need a tip selection algorithm as in IOTA, since the places where a node can append data are already tightly restricted, since a new version can only be appended on the previous version
and acknowledgements can only be appended on the new block in addition to at least one randomly chosen other block. Therefore, the Tangle necessarily represents the logical structure of the data.\\

An example of a data exchange in TCN looks as follows: a client requests for a large NDO using an ICN Interest packet and the content identifier of the NDO. 
As it is a large NDO separated into several chunks, the client receives a Manifest file representing a part of a Tangle. 
The client uses the chunk information provided in the Manifest to request for each chunk of the NDO.
Tangles are stored in a dedicate Manifest Synchronization Table (MST) data structure instead of being handled as a typical content object in the ICN forwarding plane.
This has two reasons: (i) it allows to identify and operate on Tangles (e.g., synchronize its content due to updates), and (ii) avoids eviction of Tangles in the node cache according to its cache management policy.
When a forwarder stores a Manifest representing a core element of a Tangle in its \emph{MST}, it will append an acknowledgement block to each element that it could verify.
Verification takes place during forwarding the data chunk by comparing the hash value of the signature of the chunk packet with the signature hash value present in the Manifest.
The verification degree of a core element is the number of incoming edges, which represents the number of nodes which acknowledged to a core element.
The moment a forwarder will append an acknowledgement to a core element, the other nodes storing the manifest will synchronize the change. 
We refer to this situation as Tangle synchronization.
The more forwarder acknowledge to a core element the better in order to reach consensus on the Tangle.

%In addition to improve the performance of the ICN forwarders for large NDO queries, the TCN architecture introduces a Manifest Synchronization Table (MST) as an additional data structure. 
%In the TCN forwarding plane, Tangles are stored in a dedicate MST data structure instead of being handled as a typical content object in the ICN forwarding plane (cf. Figure~\ref{fig:TCNArchitecture}).
%This has two reasons: (i) it allows to identify and operate on Tangles (e.g., synchronize its content due to updates), and (ii) avoids eviction of Tangles as potentially happen when handled in the ICN content store due to cache %management policies.

\begin{figure}
    \centering
    \includegraphics[width=.45\textwidth]{Figures/tcn_tangle.pdf}
    \caption{A Tangle consisting of \emph{core} (\textcolor{green}{green}) and \emph{acknowledgement elements} (\textcolor{red}{red}) which identify chunks (\textcolor{gray}{gray}) by hashes. Verification degree is the weight of the edges.}
    \label{fig:CoreElementTangle}
\end{figure}

\subsubsection{Linear vs. Tree Tangles}
Tangles can be modeled in different ways. 
Besides modeling a Tangle in a linear fashion where one element follows each other, the concept of Tangles also allows to model a hierarchical tree.

Instead of creating one ICN Manifest file describing the entire Tangle, e.g., by listing all core and acknowledgement elements in one Manifest, a publisher can create a Manifest file for each core and its associated acknowledgement element. 
As a result, elements of a Tangle are treated and transferred in the network as NDOs in ICN, allowing for new opportunities to handle data in TCN.

This is an important aspect, as additional nodes can contribute to the overall Tangle besides the original content publisher. 
For example in the \emph{electronic horizon} use case (cf. Section~\ref{sec:use_cases:automotive}), other nodes can improve the overall quality of the use case application by updating the Tangle with additional data sources dynamically (e.g., feeds of cameras deployed at buildings recording a hazardous situation in the vicinity). 
Being able to verify how many different nodes participated in the Tangle so far, either by creating new core elements or acknowledgements, a node knows how well certain NDOs are verified and which elements have been created by the originator and which parts have been appended by other nodes (e.g., Figure~\ref{fig:CoreElementTangle}). 

%Beside having a linear Tangle, where one element follows each other, it is also possible that an element has two or more successor and the Tangle of core elements forms a tree. 

%A content publisher will first create the Tangle of core elements. This way, the content publisher provides a manifest which is encode into a manifest file and contains all information a client needs to fetch the entire or parts of the content. For the network, a manifest file is the same as any other NDO. 

%While a client fetches the manifest and the chunks of an NDO, the nodes in the network store the manifest in the \emph{MST} and the chunks in the \emph{CS}.
%When a node stores a manifest in the MST it will append an acknowledgement block to each element that it could verify. A node can verify an element, when 
%it has the manifest and the chunk available to verify the hash of the chunk and compare it with the manifest. 
%An acknowledgement is always appended to two elements it verifies and an acknowledgement can also verify other acknowledgement.
%The moment a node will append a acknowledgement, the other nodes storing the manifest will synchronize the change. 
%As more acknowledgement pointing directly or indirectly onto an core element, as better verified it is. 
%This is important, because this way, nodes beside the original content publisher can append core elements to the Tangle and help the data to evolve. The verification degree of an core element is the number of incoming edges, which represents the number of nodes which acknowledged an core element. By checking how many different nodes participated in the Tangle so far, either by creating new core elements or acknowledgements, a node knows how well certain data are verified. In Figure \ref{fig:CoreElementAckTangle} an example for a Tangle manifest including acknowledgements is shown.

%By checking the signatures of the individual core elements, a node can always verify, which part of the data was created by the original publisher and which parts were appended by other nodes.

%\begin{figure}
%    \centering
%    \includegraphics[width=.5\textwidth]{Figures/CoreElementAckTangle.pdf}
%    \caption{A Tangle consisting of \emph{core elements} and \emph{acknowledgements}. Verification degree is the weight of the edges. For clarity we hide the chunks from this figure.}
%    \label{fig:CoreElementAckTangle}
%\end{figure}

\subsubsection{Handling Versions of Data in TCN}
According to the design rationale of immutable content identifiers in ICNs (e.g., Zhang et al~\cite{zhang2014named}), any change of the payload of a NDO results in a new version of the NDO, announced in the network using a new content identifier.
In order to be able to request for different versions, TCN's Tangles support versioning by appending new versions of individual chunks to the existing Tangle.
Instead of re-creating the entire Manifest, i.e., as in FLIC~\cite{tschudin2016file}, only the changed elements within a Tangle need to be updated, pointing to the new version of the NDO.
%As potentially each NDO chunk is represented as a Tangle element to ensure a high degree of flexibility in managing those chunks, versioning helps to manage only changed chunks and their Tangle representatives, instead of re-creating the entire Manifest structures, e.i., as in FLIC~\cite{tschudin2016file}. 
%Thereby, any node processing the chunk, whether the originator or any other entity, can add additional content to new versions of existing chunks. 
As a result, TCN allows to represent data in the network in a \emph{distributed database} fashion instead of a simple \emph{key-value store}.

However, a new version cannot be accepted without the consensus of other nodes in the network.
Whenever a change happens in a Tangle, a new version is created and appended to the Tangle, visible as history for all other nodes.
Similar like in Blockchain, all transactions on the Tangle are stored within the Tangle itself.
While a Blockchain represents a single decentralized data structure containing all content, replicated by every participant, TCN introduces decentralized data structures on each NDO.
As a result, the overhead of synchronizing new content is expected to be fewer compared to a Blockchain structure. 
Furthermore, Tangles provide more flexibility in selecting the content to be synchronized.
Staled information of a Tangle can be dropped by the publisher (e.g., non-valid version), instead of replicating all existing content as prescribed by a Blockchain.

In order to get a new version accepted in the network, a producer needs to select two core elements of a Tangle to append the new version to (cf. Figure~\ref{fig:CoreElementTangleAppend}).
We recommend that the primary element is selected in a semantic manner: if a new version of a chunk is added, it has to be appended to the block containing the previous version. 
If a chunk is replaced entirely by a new block, it has to be appended to the end of the Tangle representing the latest version.
The secondary element is selected randomly as each element at least has to point to two predecessors. 
A random selection minimizes the risk of circling pointers which increase the processing time of the entire Tangle.

%To append a block with a new chunk reference on the Tangle Manifest, a node needs to choose two Tangle elements where to append the new block. The first element is chosen in a semantic manner, so if a new version of a chunk is added, the new block should be appended to the block containing the previous version, and if a completely new chunks is added, the block with the  reference to the new chunk is added at the very end of the Tangle (which means to the latest version of the last chunk). 
%The second element is chosen randomly. Each new element will always verify two predecessors. 

\begin{figure}
    \centering
    \includegraphics[width=.45\textwidth]{Figures/tcn_tangle_version.pdf}
    \caption{A new version $core_{2.1}$ is appended to the Tangle. Core elements have a primary hash pointer on the direct predecessor (here \textcolor{blue}{blue}).}
    \label{fig:CoreElementTangleAppend}
\end{figure}


\subsection{Tangle Representation in ICN}
\label{sec:Binary_Tangle_Representation}

In order to be able to transfer Tangles in the network, an explanation of representing Tangles in ICNs follows.
Instead of representing an entire Tangle as an application data unit in an ICN, each element of a Tangle is represented as a NDO.
It allows to fetch/synchronize parts of a Tangle instead of requesting for the entire one.

As mentioned in Section~\ref{sec:tangle:design}, a Tangle is given as a list of individual blocks, while each block contains at least two pointers to previous blocks in the structure -- the primary and secondary pointers.
The following listing illustrates the structure of a Tangle element in TCN:

{\scriptsize
\begin{lstlisting}
{
    type: <core, acknowledgement>
    chunkname: <name>,
    primaryhash: <hash>,
    secondaryhash: <hash>,
    ...
    signature: <signature_of_origin>
}
\end{lstlisting}}

When creating an acknowledgement element, there is no primary hash to be defined as the element represent meta-information.

Each element of a Tangle is transferred in the network as individual NDO and accessible in the underlying ICN using a content identifier.
In TCN, we propose the following naming structure to access an element of a Tangle:

{\footnotesize
\begin{verbatim}
    <NDO-Tangle-name>/<hash-value>/<version-number>
\end{verbatim}}

The structure allows to provide fine-grained access to a Tangle element, e.g., to a particular version.
The name of the actual chunk can be chosen according to the permitted name space.

%After presenting the logical discussion of a tangle, in the following we will explain how the Tangle is mapped into network packets so that it can be synchronized. Thereby, we distribute the tangle over different elements, so that it is not required to synchronize the entire tangle. 

%The Tangle itself is just a list of individual blocks, each block contains two signatures of previous blocks.
%However, for core elements, one of the two hash values of a previous blocks is marked as primary hash. This is the hash which points on the direct predecessor, while the other hash points on a block randomly chosen. For acknowledgements there is no primary hash, since they are not used to represent data\ref{fig:CoreElementAckTanglePrimaryHash}.   
%\begin{figure}
%    \centering
%    \includegraphics[width=.5\textwidth]{Figures/CoreElementAckTanglePrimaryHash.pdf}
%    \caption{Core elements have a primary hash pointing on the direct predecessor, while acknowledgements point on two random chosen elements. \DENNIS{Can we merge content from Figure~\ref{fig:CoreElementTangleAppend} and Figure~\ref{fig:CoreElementAckTanglePrimaryHash} as they look similar??}}
%    \label{fig:CoreElementAckTanglePrimaryHash}
%\end{figure}

%Each block is stored an individual NDO. These packets are identified by their hash value, thus the name of a packet containing a block is:  
%\begin{verbatim}
%    <NDO-name>/<hash-value>/<version-number>.
%\end{verbatim}
%The name of the actual chunk to which a block is referring to can be chosen freely within the permitted NDN name space. 

%We encode the blocks using the JSON format into a binary packet, which enables easy encoding and extension. \DENNIS{BJSON??}
%A common core element block in TCN would look like the following when binary encoded: 
%{\small
%\begin{lstlisting}
%{
%   type: core
%    chunkname: <name>,
%    primaryhash: <hash>,
%    hash2: <hash>, 
%    signature: <signature>
%}
%\end{lstlisting}}
%A acknowledgement looks very similar, but the field \verb|primaryhash| is just called \verb|hash1| and the value of the field \verb|type| is: \verb|ack| instead of \verb|core|.


%Each node synchronizing the tangle maintains a list of \emph{heads}. A \emph{head} is a Tangle element with no incoming edge. This list is stored in a NDO, too.
Each time, a new element is added to the Tangle, a new version is created and appended as the \emph{tip}.
As \emph{tips} always represent the starting point for synchronizing a Tangle, the proposed naming convention to access the \emph{tip} of a Tangle is:

{\footnotesize
\begin{verbatim}
    <NDO-name>/<version-number>.
\end{verbatim}}

In order to ensure to receive the latest version from the origin, a consumer node has to specify a cache bypass signal as part of the request (e.g., ''\texttt{must-be-fresh}'' flag in NDN). 
%Since the heads are the starting point to fetch the tangle which is the manifest of the actual data, the heads have the name of the actual data. 

%Within the head element we encode the list of heads just as binary, comma separated values since no advanced structure is required. In case the list of concatenated hash values gets to long, the NDO is split into %several chunks which are enumerated. A chunk is named as following: 
%\begin{verbatim}
%    <NDO-name>/<chunk-number>/<version-number>.
%\end{verbatim}
%To identify the last chunk, the \emph{FinalBlockId} bit is set.

==> Tangle Centric Networking/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this paper, we present the challenge of tight name-to-data binding in ICNs, especially for scenarios in which Manifest solutions are used.
To address the limitations of the tight coupling, we present Tangle Centric Networking, a network level consensus and synchronisation extensions for ICNs.
In TCN, the Manifest of each NDO is represented as a Tangle, that enables the network to add or update content across multiple consumers in a distributed fashion.

We implemented the concept of TCN in simulation and compared it against the ICN Manifest solution FLIC.
The results show that Tangles provides an efficient way to synchronize immutable and mutable state over the network, while the additional synchronization overhead is negotiable when popular large files frequently change in the network.
Therefore, TCN and its Tangle concept improves the performance of data retrieval for these types of data in an ICN.

As we move toward a distributed edge computing environment, we discuss the concept of TCN as a promising extension to manage compute-centric networking architectures more efficiently.
Future work of TCN has to address the presented open directions, especially these points regarding security and trust management.



==> Tangle Centric Networking/conferencedata.tex <==
%%
%% \BibTeX command to typeset BibTeX logo in the docs
%\AtBeginDocument{%
%  \providecommand\BibTeX{{%
%    \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

%% Rights management information.  This information is sent to you
%% when you complete the rights form.  These commands have SAMPLE
%% values in them; it is your responsibility as an author to replace
%% the commands and values with those provided to you when you
%% complete the rights form.
%\setcopyright{acmcopyright}
%\copyrightyear{2021}
%\acmYear{2021}
%\acmDOI{10.1145/1122445.1122456}

%% These commands are for a PROCEEDINGS abstract or paper.
%\acmConference[submitted to: ACM ICN '21]{submitted to:  ACM ICN '21: 8th ACM Conference on Information-Centric Networking}{Sep 22--24, 2021}{Paris, France}
%\acmBooktitle{Preprint}
%\acmPrice{15.00}
%\acmISBN{978-1-4503-XXXX-X/18/06}


%%
%% Submission ID.
%% Use this when submitting an article to a sponsored event. You'll
%% receive a unique submission ID from the organizers
%% of the event, and this ID should be used as the parameter to this command.
%%\acmSubmissionID{123-A56-BU3}

%%
%% The majority of ACM publications use numbered citations and
%% references.  The command \citestyle{authoryear} switches to the
%% "author year" style.
%%
%% If you are preparing content for an event
%% sponsored by ACM SIGGRAPH, you must use the "author year" style of
%% citations and references.
%% Uncommenting
%% the next command will enable that style.
%%\citestyle{acmauthoryear}

==> Tangle Centric Networking/content.tex <==

%% -------------------------
%% SECTION 1 - INTRODUCTION
\input{introduction}

%% -------------------------
%% SECTION 2 - Use Cases
\input{use_cases}

%% -------------------------
%% SECTION 3 - Background
\input{background}

%% -------------------------
%% SECTION 4 - Concept
\input{concept}

%% -------------------------
%% SECTION 5 - TANGLE SYNC
\input{tangle_sync}

%% -------------------------
%% SECTION 6 - EVALUATION
\input{evaluation}

%% -------------------------
%% SECTION 7 - TFN
%\input{07_tfn}

%% -------------------------
%% SECTION 8 - DISCUSSION
\input{discussion}

%% -------------------------
%% SECTION 9 - CONCLUSION
\input{conclusion}

==> Tangle Centric Networking/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

In IOTA, Tangles offer a lightweight solution to handle data of IoT scenarios in a distributed manner, while not relying on concepts such as proof-of-work or a transaction fee as Blockchain.
By providing additional features such as consensus between partner nodes as well its conceptual fit to the proposed structure of Manifests as in FLIC~\cite{tschudin2016file}, TCN overcomes the limitations of tight name-to-data coupling.
These properties makes TCN an interesting candidate for distributed applications deployed especially in edge computing environments.
However, there are additional aspects of TCN not addressed so far.


%Tangles are a lightweight consensus mechanism, since they do not require a proof-of-work or a transaction fee as blockchain and said to be good for IoT. 
%In this paper we used tangles for synchronization over a NDN.
%First, TCN is not the first synchronization mechanism for NDN, since ChronoSync~\cite{Zhu:ChronoSync:2013}, pSync~\cite{Zhang:PSync:2017} and others are existing already for some time. Compared to ChronoSync. %pSync and TCN support partial synchronization. 
%However, TCN additionally supports consensus between all syncing parties, which version is the latest. Moreover, in common NDN-Manifests such as FLIC~\cite{tschudin2016file} it is required to recompute a %manifest when data are updated or append. TCN supports extensions without creating new manifest files and does not relay on a permanent network connection. A node can always work on its local tangle and %synchronize it as soon as a network connection is available, where conflicts are resolved by the tangle consensus. 
%This property makes TCN very interesting for distributed distributed applications such as chat,  distributed databases and network computing. 
%TCN supports chat applications in the same way as ChronoSync~\cite{eligar2020analysis}.  
%A distributed database would not only sync the tangle representing the manifest but also the data the individual blocks point to. This way, all nodes will end up with eventually consistency. 

\subsection{TCN -- Security \& Trust}
The current design of TCN allows easy participation of nodes on the Tangle structure.
Every node which is able to synchronize a Tangle is able to append data to it, even malicious one, due to a missing concept for authorization. 
However, similar as in Blockchains, Tangles establish a trust model based on consensus. 
Data will only be synchronized if an element is acknowledge by subsequent elements.  
Elements which get significantly less acknowledgements will be dropped from the Tangle after some time (Tangle convergence), while verified elements remain in the Tangle. 
%Moreover, especially, for applications such as distributed databases, only specific nodes are allowed to append new blocks. This can be enforced by requiring blocks to be signed by a node with permissions, otherwise, the nodes will immediately drop the block. 

As in ICN every node is required to sign a content packet, signatures within the packets might be used to authenticate a node against a Tangle.
Additional mechanisms to handle permissions to operate on the Tangle can help to prevent a node publishing malicious data.
%nodes publishing malicious data can be easily identity an even excluded. This can be done by adding a branch to the tangle, which contains the keys of malicious nodes, who's data should be ignored. What malicious data is and which nodes are banned is decided by the consensus in the tangle by all other participating nodes. 

%Finally, we can say that TCN comes with the same signing and validation process as NDN but extends it by a consensus mechanism.

\subsection{TCN -- Intelligent Cache Management}

The information modeled within a Tangle can be used for cache decision making.
A node synchronizing a Tangle can anticipate the next data chunk to be requested by a consumer node, pre-fetching and storing it within its local cache pro-actively.
As a result, TCN forwarding nodes turn into data repositories.
Such feature might be useful in time-sensitive use case scenarios such as connected vehicles~\cite{scherb2019data}.
For example, proactively storing data at edge nodes, e.g., traffic information about a hazardous situation ahead, improves data dissemination in mobile scenarios.
Furthermore, as Tangles allow to append data to an existing structure, vehicles can append own generated data or even carry data to areas not covered by a communication infrastructure, and thus, contribute to  improve the quality of the distributed application. 

%Synchronizing the tangles enables nodes to be aware of all data versions in the network. Based on this knowledge, it is possible to pre-fetch data and to keep the latest version of data objects in the cache. This changes properties of a forwarder and transforms them more towards a repository. Thus, TCN can be used to build distributed repositories and for on demand deployment of additional capacities.
%This can be useful for building content delivery networks with low latency, e.g. by synchronizing data into different regions in advanced. For example, for vehicular scenarios the pre-fetching of traffic data to edge-computing nodes can be important since they need to be available with very low latency. Moreover, the data need to be updated form the data source, since the latest traffic data are required. TCN is an optimal basis for those kind of scenario. Even more, since every node can update data, vehicles can append their own collected traffic data easily. 
%Other cars can verify the data and establish a group trust. 
%Since vehicles can also synchronize the tangle and store the data locally (on the vehicle), they can transport information into areas without infrastructure and other vehicles can synchronize and update the data. 
%Thereby, the group trust and verification degree in the tangle can help other vehicles to understand the reliability of the data. Thus, this discussion shows that TCN brings a lot of advantages into the use-case (cf. Section \ref{sec:use_cases:automotive}) described in this paper and solves its challenges. 


\subsection{TCN -- Flexible Name-to-Data Binding}
%update manifest entry, same name, different hash possible by consensus. by iterating manifest tangle, you can choose based on hash value.                        

ICNs tightly couple content identifier and actual data.
The mandatory signing procedure of ICNs ensures that these bindings can be verified at client side (or even forwarder) by relying on a Public Key Infrastructure (PKI).
New or updated content has to be published using a new identifier.
Especially, Manifest solutions like FLIC require to re-create its entire structure in case of any changes.
TCN revises the tight coupling as Tangles allow to extend the existing structure by adding new content to the Tangle on demand.
The acknowledgement mechanism of Tangles helps to establish consensus on valid elements, while less valid content will be evicted from the Tangle from time to time.
As a result, data can be enhanced not only by the originator of the data which is essentially different compared to plain NDN solutions.
To this end, TCN moves management complexity from the application level into the Tangles enabling the support of cooperative application.


%NDN is based on a strict name data binding, to update data, a new version needs to be created. Especially, in cases where manifests like FLIC are used, updating versions means often recomputing large parts of the manifest. 
%Moreover, dealing with versions can increase the overhead in an application. 

%TCN breaks off some of this. The tangle-based manifest can be extended by adding new blocks and the consensus given by the tangle is helping to decide which is the latest version. Thereby, compared to other NDN solutions 
%the decision can be decentralized and not only central by the original author of the data. This way, TCN adds flexibility to support cooperative apps directly by the network and removes complexity from the application level.

% DENNIS: IMO das ist ein eher schwaches Argument. Da TCN auf ICN basiert hast du zwingend eine PKI mit im System, dass du jetzt absichtlich bei den Tangles nicht nutzt? Und wie würde das dann funktionieren, wenn ein neuer Name zu einem neuen Objekt veröffentlicht wird. Muss dann ein Tangle ebenfalls den weg über eine PKI gehen um DATA packets zu signieren? Wo kommt das schlüsselmaterial her?

%The advantage of TCN here is, that the network agrees on which name-to-tangle (name-to-manifest) binding is valid. Attempts to change this binding will directly be rejected by the network consensus. 
%In NDN, a packet is verified by a signature and a Public Key Infrastructure (PKI) is used to verify the name-data binding on clients (or sometimes on forwarders). Thus, NDN can also reject
%NDO where the name is not signed by the owner. 
%However, in NDN this requires the PKI while TCN offers the same feature in a decentralized way, which is for example for IoT very interesting. Moreover, the decentralized approach of TCN does not prevent different users 
%to participate in the content crafting, while in pure NDN only the owner of the \emph{Private Key} can extend or update data.



%\begin{itemize}
%    \item For each chunk of an NDO, TCN recommends to introduce an Tangle element. Pros: %achieving flexibility in link and operate on individual chunks of an NDO; Cons: for each chunk %of an NDO, TCN introduces another NDO for a tangle element as well as a new name $->$ twice the %number of NDOs in the network.
%\end{itemize}
%block certain content providers. detect malicious publisher and clean data of potential %malicious chunks including caches

%Network as distrubuted database. Auto replication etc....

%advantages tangle over crdt, what can we do more

%why do core element need mandatory point on one of their predecessors

%data retrieval. data/compute graph, try to optimize this graphs, sync of compute graph, better management of network

%instant messaging. maybe easier with tangles, voip

%late sync. when a node was offline for some time


\subsection{TCN -- Towards Compute-Centric Architectures}

The introduction of TCN have shown improvements via network level consensus and efficient management of data chunks (cf. Section~\ref{sec:evaluation}).
However, the concepts of Tangles are promising for compute-centric architectures such as Named Function Networking (NFN)~\cite{sifalakis2014information}, 
named function as a service (NFaaS)~\cite{krol2017nfaas}, or Compute First Networking (CFN)~\cite{krol2019compute} as well.
For example, the \emph{electronic horizon} application logic can be modeled as a compute graph using Tangles.
By doing so, the Tangle can be synchronized between execution nodes to coordinate the execution of computations across cloud and edge environments, and thus, ensure to fulfill application demands. 
Further application domains which might benefit from such concept include distributed database systems, or distributed chat applications like Scuttlebutt~\cite{tarr2019secure, scherb2021scoiot}.
We briefly discuss the potentials of the future work on Tangle Function Networking (TFN) -- an extension of TCN supporting the coordination of computation state across multiple execution nodes in a distributed and transparent fashion.

%TCN has the potential to be used in various applications by providing a single solution for various problems.
%In the following we discuss applications which can be build on top of TCN such as a distributed database, chats-application with
%offline support and in-network computations. 

%\subsubsection{Distributed Database}
%Synchronization and Consistency is one of the key properties in distributed databases. TCN itself is, when synchronizing
%over multiple nodes a distributed database which uses a lazy replication of data. In a TCN based database, elements could be
%appended by any node, and the overall consensus will decide which data are valid and which data are not. By default, adding
%but two versions of the same same object leads to branches in the tangle. However, since both objects may be valid, either,
%one of the nodes need to re-append its data on the better verified branch, or a mergeblock needs to be appended an approved.
%A mergeblock verifies on two branches and combines both updates. A mergeblock can be issued by any node in the netwwork and needs
%to be verified such as any other block. 

%\subsubsection{Chat Application}
%TCN brings properties of which chat applications and other point to point application can benefit from. The synchronization
%of the tangle can help exchanging messages, when all participants are synchronizing the tangle. Moreover, if a node was offline,
%the messages can be added later. Therefore a chronological tangle traversal method is required. This could be done by adding timestamps
%Another advantage of the tangle is, that the synchronized tangle is offline available, similar as the log in Secure Scuttlebutt~\cite{tarr2019secure}.
%Thus, synchronized content can easily accessed offline. Moreover, Tangles do not require to keep all content stored forever,
%but only synchronizing the latest data is possible. Thus, building chat applications and social networking applications based 
%on TCN is an very interesting idea. 

\subsubsection{Tangle Function Networking}
NDN has been proven by several applications to be a good basis for network computing. NFN~\cite{sifalakis2014information, scherb2016packet}, 
NFaaS~\cite{krol2017nfaas}, CFN~\cite{krol2019compute}, etc are examples for 
network computing frameworks for NDN.
When looking into the concepts of NFN and NFaaS, it can be seen that both support the execution of stateless functions as in the ''function-as-a-service'' paradigm.
Besides stateless functions, CFN supports the execution of stateful Actors by synchronizing compute state using CRDTs.
Instead of using CRDTs, Tangles can be used for the following reasons: (i) allow for collaborative resolution of execution nodes, and (ii) allow to dynamically extend the graph by other nodes during runtime (e.g., to store and synchronize local variables and intermediate results).

A Tangle in TFN consists of two blocks: \emph{functions}, and \emph{data} (input, compute state or compute result), therefore, supports both stateless functions and stateful computations (cf. Figure~\ref{fig:TFNComputeGraph}). 
Each of these blocks are represented as individual elements in the Tangle.
When an execution node parses the Tangle, it can decide to execute a function of the graph.
Pointers to additional information such as the location of the function executable, as well as further data is available in the Tangle as well.
In case a compute result is available, the Tangle is updated accordingly that subsequent execution nodes can query quickly the network for the result.
Furthermore, modeling a compute graph using Tangles allows for parallel processing of the entire graph.
In case multiple execution nodes are involved in the overall computation, a node takes over responsibility to execute a function by acknowledging the execution in the Tangle, and synchronized partners will be notified accordingly. 
Furthermore, it limits the probability that a function within the Tangle is executed in parallel by different nodes.

As we move toward a distributed edge computing environment, the concept of TCN is promising for compute-centric networking architectures~\cite{scherb2018smart, scherb2019execution}.
It allows the compute network to change or extend computation graphs during the runtime, bringing more flexibility than all other computation frameworks introduced so far~\cite{scherb2017execution}.
For example in the \emph{electronic horizon} scenario (cf. Section~\ref{sec:use_cases}), to warn the driver about a hazardous situation on the junction ahead, nodes can append image processing computations of a camera deployed close to the junctions to the compute Tangle or append the processing result to the Tangle as additional input for the computation~\cite{scherb2018resolution, grewe2018network}.
Another promising feature, especially in mobile scenarios is the capability that Tangle-based computations can be continued offline in case of connection loss.
%After re-connecting to the network, 
%This makes the TFN concept also very interest for swarm computations, where nodes join an leave.

%The tangle of TCN can be used to represent a computation graph and to store and synchronize local variables and intermediate
%results. Thus, building a computation framework on top of TCN is another possibility to execute computation in NDN.
%A computation framework on top of TCN is called Tangle Function Networking (TFN). 
%The tangle based computation graph representation in TFN has an important advantage. It enables the network to change or extend
%computation during the runtime bringing more flexibility than all other computation frameworks in NDN. Moreover, the tangle 
%based computation can be continued offline in case of connection loss. This makes the TFN concept also very interest for
%swarm computations, where nodes join an leave. 

%The tangle based compute graph in TFN consists of two blocks: \emph{functions}, and \emph{data} (input, compute state or compute result). Each of these blocks are represented as individual elements in the Tangle %(cf. Figure~\ref{fig:TFNComputeGraph}). 
%For example, an element for a function call is used to instantiate a function and contains a pointer to the executable (byte code) of the function to be fetched by other nodes if not already present.
%Examples of a \emph{data} element representing a compute state can be the value of a variable in the compute stack or an intermediate results which dependent on computation state or the data to be synchronized %across multiple execution nodes. 
%Therefore, TFN supports stateful computations.
%In case a compute result is available in the network, the Tangle is updated accordingly that subsequent consumer can quickly query the network for the result.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/TFNComputeGraph.pdf}
    \caption{Compute Graph of the function call \texttt{func1(func2(data3),data1)} in TFN. This figure shows only logical compute graph excluding the second hash reference of the tangle.}
    \label{fig:TFNComputeGraph}
    \vspace{-0.5cm}
\end{figure}

%While a Tangle in TFN allows to model coordination of the execution of functions, coordination strategies are required to decide which node computes which part of the overall computation.
%To simplify TFN, we propose to use one of the existing solutions of existing compute-centric networks. 
%For example, NFN provides several strategies according to the scenario (e.g., mobility~\cite{scherb2019execution}, or \cite{scherb2018smart} for long running computations), while CFN provides task scheduling to %coordinate functions across worker nodes~\cite{krol2019compute}.
%However, a Tangle can be used to model the compute flow of the overall computation as well. 
%Compute nodes can already commit to execute a function using an acknowledgement and start to execute the function if the required data (e.g., intermediate result) is available in the network.

%The concept of Tangles allows extensions to the data structure during runtime. In TFN, this allows to modify the compute graph dynamically, e.g., to adapt to long running computations. 
%For example in the \emph{electronic horizon} scenario (cf. Section~\ref{sec:use_cases}, to warn the driver about a hazardous situation on the junction ahead, nodes can append image processing computations of a %camera deployed close to the junctions to the compute Tangle or append the processing result to the Tangle as additional input for the computation.
%Any node synchronizing the Tangle is able to verify the new element and accept or reject it. In case such element is accepted, everyone subsequent node benefits from the additional computation result which is %produced. In case the element got rejected, the original Tangle remains in tact, and therefore, the applications using its compute result.


%Furthermore, modelling a compute graph using Tangles allows for parallel processing of the entire graph, depending on the type of application.
%In case multiple execution nodes are involved in the overall computation request, a node acknowledges the execution of a function and updates the Tangle accordingly (cf. Figure~\ref{fig:TFNComputeGraph}, \emph{computing-this}-note). 
%This procedure allows to coordinate the execution of the entire compute graph across multiple execution nodes transparently and in a distributed fashion. For example, in case a node joins the overall computation process after a connection loss, it has to synchronize only the remaining parts of the overall computation graph to fulfill its contribution. Previous compute states, as labeled by acknowledgements in the Tangle, can be ignored.
%Furthermore, it limits the probability that a function within the Tangle is executed in parallel by different nodes.

==> Tangle Centric Networking/evaluation.tex <==
\section{Evaluation} %TODO eval nach oben
\label{sec:evaluation}

In order to evaluate the scalability of TCN, the networking simulator NS-3~\cite{ns3:2018} and the NDN specific protocol stack bundle ndnSIM 2.7~\cite{ndnSim:2017} are used to create the simulation.
Dependent on the number of synchronization nodes, the time required to synchronize to parts as well as a full Tangle is compared against the FLIC Manifest proposal.

\subsection{Synchronization}
As topology for our simulation we use the rocket-fuel typology~\cite{spring2002measuring}\footnote{more specific the \texttt{1221.cch} based on \url{https://github.com/cawka/ndnSIM-sample-topologies}} including 2766 nodes with a bandwidth capacity between $2$MBps and $10$MBps, representing a hierarchical network as shown in Figure~\ref{fig:rocketfuel}. We run the evaluation $100$ times and every time we initialized the bandwidth capacity of the links differently.
\begin{figure}
    \centering
    \includegraphics[width=.4\textwidth]{Figures/rocketfuel.pdf}
    \caption{Rocketfuel Topology with 2766 nodes, visualized with pyviz in ndnSIM.}
    \label{fig:rocketfuel}
\end{figure}

To evaluate the scalability of TCN, we choose randomly $n$ nodes (range: $n=4$ up to $n=256$) to be involved in the procedure. 
The size of the NDO to be modeled as a Tangle is $1$GB, while each chunk is of size $50$KB. 
Based on these parameters, the Tangle to be simulated consists max. of $20973$ blocks. 
In the Tangle bootstrapping, all $n$ nodes synchronize the content of the Tangle. 
Afterwards, nodes will start to append new chunks of max. size $200$MB to the Tangle (max. $4096$ additional blocks in total).
We measure the time taken to synchronize the entire Tangle at every participating node. 
Moreover, we request the actual data and measure the time until all nodes have fully synchronized to the desired data.
The bandwidth is randomly chosen per link, between $2$MBps and $10$MBps.

We simulate the scenario either using FLIC and a full-synchronization of a Tangle. 
The results are illustrated in Figure~\ref{fig:sync}. It can be seen that FLIC requests the entire Manifest again when a change happend in the NDO. 
When looking at the synchronization time, it can be seen that TCN has a rather constant time saving compared to full synchronization in FLIC.

\begin{figure}
    \centering
    \includegraphics[width=.4\textwidth]{Figures/sync.png}
    \caption{Result of full synchronization using TCN and FLIC (100 runs with random bandwidth initialization).}
    \label{fig:sync}
    \vspace{-0.4cm}
\end{figure}

This is due to the fact that a fewer number of Manifest packets have to be transferred in the network as we append elements to the Tangle, while FLIC requires a re-creation of the entrie Manifest structure.
The experiment shows, that an efficient Manifest structure can help to speed up real world applications.
%Since we do not have any simulated packet loss, the number of requests per node is the number of additional chunks in TCN and the number of manifests using FLIC multiplied with the number of requesting nodes. 
The synchronization time has a roughly linear grow despite the number of nodes is exponential growing. 
This can be explained by the intrinsic multicast and in-network caching capabilities of NDN as forwarding nodes in the simulated topology will respond to synchronization requests with cached data.



In a second experiment we use the same setting, but we want to analyze the scaling behavior of TCN vs FLIC. Therefore, we change the size of the initial data to $10$, $50$, $100$, $200$, $300$, $400$, $500$, $600$, $700$, $800$, $900$ and $1000$MB
and we observe the time how long TCN and FLIC need to synchronize additional $200$MB.
The result is shown in Figure \ref{fig:Scale}.
\begin{figure}
    \centering
    \includegraphics[width=.4\textwidth]{Figures/Scale.png}
    \caption{Result of full synchronization using TCN and FLIC with different file sizes.}
    \label{fig:Scale}
    \vspace{-0.5cm}
\end{figure}

We see that for small data ($10$, $20$, $50$MB) TCN and FLIC have a rather similar performance. However, with increasing file sizes, full synchronization with FLIC as manifest becomes slower than TCN due to the overhead of requesting the entire manifest compared to TCN only fetching the new blocks. Thus, we find that with increasing file size TCN scales very well. This is important, since when the amount of synchronized data grows, the synchronization overhead should not increase for optimal performance. 


%\subsection{Connection Loss}
%One of the key properties of a tangle is, that even without network connection, tangles can be extended. We use a four by four grid and disable randomly nodes. While being disabled the nodes can still append data to its own tangle. The moment the node come back online, it can update its %own tangle and other nodes can fetch updates. This will create a separated path in the tangle for the data of the disconnected node.  

==> Tangle Centric Networking/header.tex <==
%%
%% The "title" command has an optional parameter,
%% allowing the author to define a "short title" to be used in page headers.
\title{Tangle Centric Networking}

%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.
\author{Christopher Scherb}
\email{christopher.scherb@unibas.ch}
\affiliation{University of Basel, Basel, Switzerland}

\author{Dennis Grewe}
\email{dennis.grewe@de.bosch.com}
\affiliation{Robert Bosch GmbH, Renningen, Germany}

\author{Christian Tschudin}
\email{christian.tschudin@unibas.ch}
\affiliation{University of Basel, Basel, Switzerland}

%%
%% By default, the full list of authors will be used in the page
%% headers. Often, this list is too long, and will overlap
%% other information printed in the page headers. This command allows
%% the author to define a more concise list
%% of authors' names for this purpose.
%\renewcommand{\shortauthors}{C.Scherb and D.Grewe and C.Tschudin}

%%
%% The abstract is a short summary of the work to be presented in the
%% article.
\begin{abstract}
Today's Internet is heavily used for multimedia streaming from cloud backends, while the Internet of Things (IoT) reverses the traditional data flow, with high data volumes produced at the network edge.
%Solutions of distributed edge computing environments support the execution of IoT applications in a decentralized and distributed manner.
%However, the underlying host-centric communication model challenges those environments on different levels.
Information Centric Networking (ICN) advocates against a host-centric communication model which is promising for distributed edge computing environments and the execution of IoT applications in a decentralized fashion. 
By using naming schemes, data is tightly coupled to names instead of hosts which simplifies discovery and access to data and services. 
However, the tight coupling challenges network performance due to additional synchronization overhead of large data volumes and services.

We present \emph{Tangle Centric Networking (TCN)} -- a decentralized data structure for coordinated distributed applications and data exchange following principles of ICN.
TCN can react on data and service changes and update them accordingly in network nodes, provide distributed data structures and enable cooperative work on the same data without huge overhead by using Tangles for coordination. We implemented TCN in simulations and evaluated the concept against a base line scenario.
\end{abstract}

\maketitle

==> Tangle Centric Networking/interactions.tex <==
\section{Interactions in TCN}

\subsection{Build-In Operations in TCN}
\label{sec:tangle:operations}

\DENNIS{STOPPED HERE}
\COMMENT{Here the sync part needs to go, we have that later in the sync section in detail}
\COMMENT{Move this behind the sync chapter}
\COMMENT{Push vs. Pull based communication in ICN - evtl. Ref to ''Mobile Data Repositories at the Edge''}

For updating the manifests, a synchronization mechanism such as PSync~\cite{Zhang:PSync:2017} or a similar synchronisation mechanism can be used. Another option is to use a
publish subscribe system where nodes holding the manifests (and so the content) subscribe to each others updates. 
By updating the manifests, the nodes see, if chunks were added to a NDO, were removed or updated. In case there were changes to chunks the node
holds, the node can update the chunks and a client will always receive the latest version. A scheme of synchronizing the MST and updating chunks between nodes is shown in Figure \ref{fig:TCNSyncExample}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/TCNSyncExample.pdf}
    \caption{Scheme of synchronizing the MST and updating chunks.}
    \label{fig:TCNSyncExample}
\end{figure}

Since the tangle representing the manifest document all changes on the chunks (and by that on the content), the network can provide functionality to
request any version of the file. A client can send the following requests to the network: 
\begin{itemize}
    \item \texttt{get(name)}: get the latest version of a NDO \\(also: \texttt{get\_latest(name)}).
    \item \texttt{get\_initial(name)}: get the initial version of a NDO.
    \item \texttt{get\_list(name)}: list all versions of a NDO.
    \item \texttt{get\_version(name, version)}: get a specific version of a NDO.
\end{itemize}

For all nodes which are synchronizing the manifest, further commands are available:
\begin{itemize}
    \item \texttt{update\_chunk(manifest\_name, chunk\_name, \\ new\_content)}: update a specific chunk in a specific manifest.
    \item \texttt{remove\_chunk(manifest\_name, chunk\_name)}: \\ remove a specific chunk from a manifest.
    \item \texttt{add\_chunk(manifest\_name, new\_chunk\_name, \\ chunk\_to\_append, new\_content)}: add a specific \\ chunk to a manifest. Append it to a specific existing chunk.
\end{itemize}

However, a command cannot be executed without the consensus of the other nodes. Whenever one of this operations is accepted, a new version
is created. This way, the file history is available to all nodes. This structure is comparable with block-chain data storage where in the block-chain only the hash value is stored, which references to the actual data. However, while a block-chain is a single decentralized data structure which is replicated by everyone, TCN brings 
one decentralized data structure per published content. Thus, the synchronization process of TCN is very lightweight compared to block-chain. Moreover, Tangles are more flexible then block-chain. They can be particularly synchronized and still be validated. More over, old stale information of the Tangle can also be dropped. 
This way, a publisher can decide to drop old versions of a file and don't need to 
continue storing all old version of a file, while nodes in the network can continue doing so. 



\DENNIS{MOVED TANGLE DESIGN UP IN CHAPTER}

\subsection{Logical Tangle Traversal}
Beside the cryptographical structure of a tangle, which is defined by which element is verified
by which other element, there is also a logical structure. The logical structure concerns the Structure
of the NDO and the chunks and is important for the node to handle requests and to perform operations on the Tangle.
The idea here is, that from the given tangle, a node creates a logical representation, so that it can easily traversal the tangle and serve requests like linear streaming or delivering a specific version of the entire NDO or of parts of it. For those kind of requests, the pure tangle structure is not sufficient, since it only allows traversing backwards. 
When a node starts synchronizing a tangle, it will store the blocks in the MST and beside it will keep create and store the logical representation for a fast reaction time.

To build the logical structure, a node will traverse the tangles from the head to the start. Thereby, it uses the property that the core elements have primary hash entries, which have a semantic meaning. Moreover, acknowledgements are not required for the logical structure of the NDO.

The goal is to create a graph that enables the node to easy traverse from the first to the last chunk in any available version of the NDO. 

Thus, the node will organize the blocks as following: Starting from the first block which references the first version of the first chunk a logical graph is created. Thereby a block points to its successor, extensions as well as to newer versions of itself. The pointers have a different type, so that when traversing the logical graph, it is easy to find elements one is looking for. 

For each version or extension of the content another pointer is added to the base version of the next block.
This way, it is fast to traverse the Tangle and to easily pick the different versions of the NDO or even of individual chunks. 

In general, this data structure is not required, since all information are stored in the tangle by using the primary hash pointer, but it is more efficient at run time to identify the relevant blocks. Figure \ref{fig:TangleLogicalStructure} shows the logical structure of a tangle as it would be used in TCN.


\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/TangleLogicalStructure.pdf}
    \caption{Logical Structure of the Tangle, which helps nodes to quickly find requested chunks}
    \label{fig:TangleLogicalStructure}
\end{figure}

%TODO, if we have space, we can talk here how getVersion etc is implemented

%TODO figures: elements and 





% TODO CHECK WHERE TO PUT THIS CONTENT??
%The manifest is stored in MST. Beside storing the manifest the MST is also synchronizing the manifests with the manifests of the same NDOs stored on different nodes. 
%In addition to improve the performance of the ICN forwarders for large NDO queries, the TCN architecture introduces a Manifest Synchronization Table (MST) as an additional data structure. 
%In the TCN forwarding plane, Tangles are stored in a dedicate MST data structure instead of being handled as a typical content object in the ICN forwarding plane (cf. Figure~\ref{fig:TCNArchitecture}).
%This has two reasons: (i) it allows to identify and operate on Tangles (e.g., synchronize its content due to updates), and (ii) avoids eviction of Tangles as potentially happen when handled in the ICN content store due to cache %management policies.

%\begin{figure}
%    \centering
%    \includegraphics[width=0.45\textwidth]{Figures/TCNArchitecture.pdf}
%    \caption{Scheme of the architecture of a TCN Node including the classic ICN/NDN forwarding pipeline.}
%    \label{fig:TCNArchitecture}
%\end{figure}

==> Tangle Centric Networking/introduction.tex <==

%\begin{comment}
%\COMMENT{
%\begin{itemize}
%    \item CRDT $->$ Tanlges, partial sync, (patrtial) result fetch from other apps due to eventual consistency and non-full sync. less interactions with other distributed applications
%    \item CRDT $->$ PSync, compute graph using psync not considered so far
%    \item Tangles $->$ PSync, results still in manifest re-creations instead of updating tangles (Proof?? how many manifests in pysnc compared to tangle)
%    \item CRDTs not optimal for long running tasks $->$ as partial computations can be published as tangles (double check CFN paper)
%    \item PSync $->$ CRDTs/Tangles, network can use tangles (or crdts) to agree on a specific name/data binding and update it.
%    \item is data flow processing with tangles possible, as in CFN not that easy to be realized $->$ fix deployment of function at flowing 
%\end{itemize}
%}

%\end{comment}

\section{Introduction}
\label{sec:intro}

% TODO Fokus auf IoT domaene da Problematik von Manifest-updates, je nach domaene, mehr gegeben ist, z.B.: automotive, industrial IoT, Vision Processing, etc.?

%As a result, research activities have focused on distributed compute infrastructures to execute applications at the edge of the network to reduce latency and data traffic %in the core network (e.g.,~\cite{Mach:MEC:2017}). 
%However, the traditional networking concepts such as a host-centric addressing scheme challenges the network at many levels. 
%Information-centric networks (ICNs)~\cite{Zhang:NDN:2014} present a promising solution with regard to consumer mobility by advocating against a host-centric communication %model. 
%The support of native network-layer ''route-by-name'' resolution simplifies the discovery of compute resources at the network edge which reduces response times significantly~\cite{Grewe:2018}.

The Internet of Things (IoT) is reversing the data flow from traditional \emph{cloud-to-edge} to \emph{edge-to-cloud} with much of the data produced at the edge.
While the number of IoT devices will double until 2025 up to 75 billion~\cite{Statista:IoT:2025}, the data produced by these devices at the edge require processing upfront before sending it towards cloud backends (e.g.,~\cite{Moustafa:rCDN:2017}).
Such a paradigm shift enables novel classes of distributed applications which are deployed in challenging environments such as highly connected automated driving, manufacturing automation or gaming.
Examples include applications demanding for timely information sharing, often to multiple consumers, which cannot be satisfied by classic cloud-based solutions.

The Edge Computing (EC) paradigm is concerned about to supporting these classes of applications. 
EC brings computational resources, storage and services from the cloud backend to the edge of the network and therefore, closer to the data origin and its consumers (e.g.,~\cite{Bonomi:2012}).
However, most of today's network architectures are still based on a host-oriented communication model, interconnecting components with each other such as the Internet Protocol (IP) technology stack.
The model challenges the network at many levels such as management and orchestration of data and services, i.e., in mobile scenarios. 
As a result, additional frameworks are introduced to manage the overhead in the communication infrastructure such as ETSI OSM~\cite{ETSI:OSM:2021} for management of services in upcoming 5G cellular deployments.
Instead, native network-layer resolution of desired data and services avoids additional communication overhead (e.g., DNS) and has the potential to reduce response times significantly. 

Information Centric Networks (ICN) present a promising solution for novel classes of distributed applications in IoT deployments (e.g.,~\cite{Amadeo:ICN:IoT:2016}).
Based on a loosely coupled communication model, ICNs use location-independent, unique \emph{content identifiers} such as naming schemes for discovering and accessing data in the network~\cite{jacobson2009networking}.
This approach couples data to an identifier instead of the host and thus avoids resolution conflicts.
It allows mobility support by nature, while not maintaining network addresses of hosts and also facilitates additional features such as in-network processing and caching of data.
Therefore, it can be a great fit to provider-agnostic distributed applications in IoT scenarios.

As ICNs target to support a wide range of distributed applications, there are special classes of application data which challenges data discovery and management,
for example, data changing at frequent intervals (e.g., a temperature sensor) as well as large volumes of data (e.g., video stream of a surveillance camera).
In order to simplify the access, ICNs propose the concept of Manifests (e.g., FLIC~\cite{tschudin2016file}). 
Manifests describe properties of a data item including a list of \emph{content identifiers} for smaller application specific chunks.

While Manifests simplify the access to special classes of application data, it introduces a challenge on the handling frequent changing data items.
Every time a data item changes, a new version of the item is created and published under a new unique \emph{content identifier}.
However, the tight coupling of data to immutable content identifiers results in frequent re-creation of the entire Manifest.
This design decision introduces the problem on how to select and announce new versions of data in the network to avoid collisions.
It either requires centralized name resolution systems managing these identifiers (e.g., NDNS~\cite{afanasyev2017ndns}), mechanisms to achieve consensus about identifiers (e.g., synchronization across nodes), or the same data is published using different identifiers, unnecessarily occupying resources, and thus, decreases network efficiency.

To address these limitations, distributed data structures offer data replication across the network. 
Examples include Distributed Hash Tables or Conflict-free replicated data types (CRDTs)~\cite{Shapiro:CRDT:2011}.
In IoT scenarios, distributed ledger technologies have gained attention in the research community in recent years.
An example to highlight is IOTA~\cite{IOTA:2021}, offering a lightweight solution to represent data in form of Tangles. 

In this paper, we propose Tangle Centric Networking (TCN) -- a network level consensus and synchronisation extensions for ICNs using Tangles~\cite{popov2018tangle}. 
Implement as directed acyclic graph (DAG), Tangles are aligned to the proposed structure of existing Manifest solutions like FLIC~\cite{tschudin2016file}, while promising additional features such as extensibility and distributed consensus.

The contributions of the paper are:
\begin{itemize}
    \item introduction of a concept of Tangles in ICNs for network level consensus and efficient management of data objects
    \item implementation and evaluation of TCN using Named Data Networking (NDN)~\cite{zhang2014named} and the PSync~\cite{Zhang:PSync:2017} protocol showing performance improvement in data retrieval
    \item discussion of further potentials and open research directions
\end{itemize}

The remainder of the paper is structured as follows: Section~\ref{sec:use_cases} introduces a use case scenario. 
Section~\ref{sec:background} provides the related work, while Section~\ref{sec:tangles} introduces the concept of TCN and certain architectural aspects in Section~\ref{sec:tangle_sync}.
Section~\ref{sec:evaluation} presents the implementation and evaluation of TCN, followed by a discussion on the results and open research directions in Section~\ref{sec:discussion}.
Finally, we conclude the paper in Section~\ref{sec:conclusion}.


%% OLD INTRODUCTION TEXT
%Modern computer networks are characterized by a large number of devices and a huge amount of data transfers caused by 
%video streaming and also by Internet of Things (IoT) devices. The focus of the network is on transferring data from
%one node to another node and often to multiple other nodes. However, the most networks architecture is still based on
%Internet Protocol (IP)-technology which was designed to connect devices to each other and not to connect user to data. 
%The way IP is often used today is that a client connects to a specific server and tells the server to deliver certain
%data. The disadvantage of this concept is that \COMMENT{management of} multicasts are complicated, caching of data close to the clients or 
%request combination is difficult to implement. \DENNIS{Dennis: Was it mit Overlay Loesungen?} Thus, usually a request is send for each client from up to the server. 
%\DENNIS{Dennis: IMO erster Absatz ist ein wenig gemischt was die Domaene angeht die du betrachtest. Ist media streaming nun eine Herausforderung, wenn ja was genau, und was ist die Herausforderung von IoT? Ggf. mit einem Beispiel wie Netflix oder vernetzte Fahrzeuge und ggf. finden wir noch ein paar Zahlen, welche die Herausforderung belegen?!}\\

%Information Centric Networking (ICN)~\cite{jacobson2009networking, zhang2014named} attempts to better fit modern use cases of computer networks by focusing on data
%instead of hosts. Host and data are decoupled. Data are identified by hierarchically names and requested by this name. \DENNIS{Dennis: Fuer NDN und CCN korrekt, aber andere archs bauen nicht zwingend auf hierarchischen namen auf.}
%Data can easily be distributed stored or cached on any node inside the
%network and be delivered from the closest location to a requesting client. This brings many advantages, since 
%multicasts become a natural part of the network and content can be secured on file instead of connection level. 
%Moreover requests can not only be requests for data, but also for computation results~\cite{sifalakis2014information}, where
%the computation workflow is encoded into the request message. 
%ICN automatically becomes more decentralised compared to TCP/IP networks, since due to naming data, DNS-like systems are not required and data can be 
%easily distributed over the network.\DENNIS{Dennis: Korrekt, aber du brauchst in ICNs auch sowas wie in name-resolution system, richtig? Eher ein schwaches als starkes Argument.}
%This makes it very usable for Internet of Things (IoT) devices \COMMENT{(e.g., Amadeo et al.~\cite{Amadeo:ICN:IoT:2016}}.

%To achieve the caching of data without conflicts, ICN comes up with a straight forward solution: Thus, all data need to be \COMMENT{uniquely} named, the name to data binding is unchangeable. 
%This requires the name to contain a version number. \DENNIS{Dennis: Nur wenn mehrere Versionen entstehen - gibt es hier evtl. Zahlen, z.B.: aus der Datenbank- oder CDN-Welt?}
%Usually, ICN structures data in chunks, which are identified by manifests (e.g., FLIC~\cite{tschudin2016file}). A manifest is basically a list
%(or a more complex data structure) of names which is used to find the names of the individual chunks. 
%To update a single chunk, the whole manifest needs to be re-created.
%\DENNIS{Dennis: Frage: Das Manifest-Update-Problem betrifft doch nicht nur Caching, richtig? Jegliche Form von Datenaustausch, sei es statisch oder dynamisch welches nicht in 1x Data packet passt. Somit ist das Problem doch viel fundamentaler als hier beschrieben?!}

%Moreover, especially caching data can lead to outdated data in the caches of certain routers. In case, the latest
%data are required, the network needs to forward a request to the data source. Therefore, to avoid fetching outdated data, 
%it is required that the network or the client understands when a data object was created and when it becomes outdated. \DENNIS{Dennis: Eher ein schwaches als starkes Argument, da es ja das ''MustBeFresh-Flag'' in NDN gibt. Liegt das Probelm nicht darin, dass Caches in sync gehalten werden muessen um populaere Daten vital zu halten?}
%When client requests the latest version of a data object, it is necessary to receive the data object from the publisher/original data source. 
%This can break parts of the caching and load balancing mechanism from ICN. For computations in the network handling the latest data
%adds additional challenges such as adding a version number to the result, since the same computation could be simultaneously executed on different
%locations and there may be no consensus about the version number.

%To handle version numbers, manifests and more complex names, NDNS can be used \cite{afanasyev2017ndns}. However introducing DNS like systems, 
%ICN becomes more centralized. \DENNIS{Dennis: Und das ist ein Problem, weil \ldots?}

%This shows the need of network level extensions for ICN for consensus about data updates, version numbers and computations. 
%Blockchain as a distributed ledger can be a way to address this shortcomings, but a single big data structure is too lazy to 
%handle huge amount of network traffic. 

%Therefore, we propose a consensus and synchronisation mechanism using Tangles~\cite{popov2018tangle}. We use one tangle per data object,
%since a tangle can be used as manifest to organize the chunks as well as a consensus and synchronization mechanism. 
%Moreover, we show, that a tangle can also be used to maintain the computation state and enable better cooperative computations in 
%Named Function Networking (NFN)~\cite{sifalakis2014information}.

%TODO Paper overview

==> Tangle Centric Networking/packages.tex <==
\usepackage{listings}
\usepackage{xcolor}% coloured text
\usepackage{hyperref}
\usepackage{graphicx}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{color}

==> Tangle Centric Networking/tangle_sync.tex <==
\section{TCN - Synchronization of Tangles}
\label{sec:tangle_sync}

The synchronization of Tangles and their contents across multiple consuming nodes in the network describes a major aspect in TCN.
For example, if a new version of a NDO is created, both the Tangle and its elements as well as the consuming nodes have to be updated to the latest version.
However, as a Tangle represents a data structure distributed across the network, it describes a non-trivial task to update records as well as to update forwarding rules to reach the latest version.

\subsection{Bootstrapping and Synchronization}
\label{sec:tangle_sync:boot}

The synchronization is separated into two parts: (i) \emph{bootstrapping} -- the initial Tangle information are requested, and (ii) \emph{synchronization} -- partial or full synchronization of a Tangle with other nodes.

\subsubsection{Bootstrapping} The Tangle \emph{tips} are ideal to bootstrap a Tangle as they represent the elements without incoming edges.
By querying the network for the desired NDO using its content identifier, a consuming node will receive the \emph{tip} of the Tangle (cf. Section~\ref{sec:Binary_Tangle_Representation}).
Starting from the \emph{tips}, the node will traverse the Tangle to the first block, requesting for all predecessor elements as well as all chunks of the desired NDO using the (primary) hash pointers provided in each element.
While traversing backwards through the Tangle, a node can already fetch the latest versions of chunks.
By evaluating the acknowledgements of the Tangle, the node can decide to fetch further elements of the Tangle, or to drop these parts.
The node will proceed the initial bootstrapping as long as all elements are received.

\subsubsection{Synchronization} 
In order to get updates on the Tangle, the node will setup a synchronization of the \emph{tips}.
This can happen either by frequently poll for new versions, or using an ICN synchronization protocol such as PSync~\cite{Zhang:PSync:2017} or ChronoSync~\cite{Zhu:ChronoSync:2013}. 
Thereby, TCN benefits from the ICN in-network caching capability for which the network will automatically store replicas frequently in forwarders to increase the availability of data in case of node failures.
In case a new element is appended to a synchronized Tangle, either a new entry is added to the list of \emph{tips} or it will be linked to a synchronized \emph{tip}. 
As a result, any updates can be quickly identified and the Tangle is synchronized accordingly. 
It has to be mentioned that the synchronization interval to be selected for a Tangle is dependent on the application type. 
The frequent data is generated or requested by the application, the shorter synchronization intervals are required.

\subsubsection{Logical Tangle Representation for Special Interactions}
Special types of application interaction patterns, e.g., streaming of data such as video, are challenging to be realized as Tangles as the pure structure only allows traversing backwards.
To overcome this limitation, a node has to create a logical representation of the Tangle in the reverse order the Tangle is traversed from the tips to the start.
When a node starts synchronizing a Tangle, it will store the elements in the MST in reversed order as traversed from the tips to the start.
The logical representation allows to identify and request for the 'next' elements of the NDO to be streamed.

%However, a consumer can not easily traverse the Tangle to request for data chunks, as the pure Tangle structure only allows traversing backwards.

%To overcome this limitation, a consuming node has to create a logical representation of the Tangle, used to easily traverse the Tangle and server requests l

%Beside the cryptographical structure of a tangle, which is defined by which element is verified
%by which other element, there is also a logical structure. The logical structure concerns the Structure
%of the NDO and the chunks and is important for the node to handle requests and to perform operations on the Tangle.
%The idea here is, that from the given tangle, a node creates a logical representation, so that it can easily traversal the tangle and serve requests like linear streaming or delivering a specific version of the entire NDO or of parts of it. For those kind of requests, the pure tangle structure is not sufficient, since it only allows traversing backwards. 
%When a node starts synchronizing a tangle, it will store the blocks in the MST and beside it will keep create and store the logical representation for a fast reaction time.

%To build the logical structure, a node will traverse the tangles from the head to the start. Thereby, it uses the property that the core elements have primary hash entries, which have a semantic meaning. Moreover, acknowledgements are not required for the logical structure of the NDO.



%For the bootstrapping process we will use the heads (the blocks without incoming edge).
%First, to start a node will request the list of heads. Starting from here, the node will request the predeceasing blocks by using the hash pointers which is used to verify the previous block. This is possible since the chunk name is given by the name of the NDO, the hash value and the version number (see \ref{sec:Binary_Tangle_Representation}).

%Thereby, all acknowledgements and blocks can be synchronized, but also only a part of them. While traversing backward through the tangle it is also possible to e.g. only synchronize the latest version of a chunk.

%As soon as all blocks are received, the node can create the logical representation of the Tangle. 
%Meanwhile, the node will setup a synchronization of the heads file. This can happen either by polling for new versions, using a known NDN-sync protocol~\cite{Shang:NDNSync:2017} such as pSync~\cite{Zhang:PSync:2017} or ChronoSync~\cite{Zhu:ChronoSync:2013}. Thereby, TCN benefits from the NDN property, that the network will automatically choose a replica, thus, if one node is interrupted, another one will be used for synchronization. 
%Any new appended element will either be directly in the heads list or it will be close to one of the heads. Thus, updates can be quickly synchronized. The synchronization interval is dependant on the application type. As more real time data are involved, as shorter synchronization interval is required. 

%After establishing the synchronization, a node can replicate the tangle. To enable the node to also add data to the tangle, it is required to also start synchronizing the other way around. 
%For this we rely on the forwarding system of NDN. 


%todo figure

\subsection{Synchronization Chain - Update Forwarding Rules}

The synchronization of a Tangle across the network requires full interconnection of subscribing nodes as potentially each participating node can add new blocks to the Tangle.
%As Tangles are eventual consistent by design (see Popov~\cite{popov2018tangle}), adding new elements to the Tangle might happen simultaneously in the network.
This situation challenges the synchronization procedure in TCN as several updates might be received in a converging node.
To overcome this limitation, TCN establishes a logical synchronization chain between participating nodes.

After a consumer bootstrapped a Tangle, it will send out a special notification message into the network to discover at least one other node synchronizing on the same Tangle, e.g., using the postfix \texttt{findsyncpartner} in the content identifier.

{\footnotesize
\begin{verbatim}
    <Tangle-name>/<nonce>/findsyncpartner
\end{verbatim}}

If the notification message is overheard by a potential synchronization partner, the partner will respond back to the notification.
This response message is processed differently by the TCN forwarding pipeline by updating entries in the forwarding table to establish a bidirectional connectivity between these nodes.
As a result, request and response messages for the particular Tangle on the network interfaces are forwarded towards the synchronization partners.
%\DENNIS{Would it not also possible to use other protocols such as RICE or R2C messages to avoid FIB manipulations?, yes, but rice manipulates the pit, i am not totally sure if that works with longest prefix matching}

To establish a bidirectional connectivity, we propose a three way handshake (cf. Figure~\ref{fig:HandshakeProcess}), so the new created FIB entries will only be persistent, if the initializing node confirms to the new routes.  
All forwarding entries created by TCN are time-limited to avoid security threats such as Denial-of-Service attacks. 
A heartbeat mechanism ensures that, in case of a timeout, FIB entries are removed accordingly.


%Synchronizing the tangle required to be fully connected, so that each node can add blocks and blocks are transferred to the other nodes. Since tangles are conflict free when adding new blocks this is not required to be in real time. 

%It is not enough to receive a head from one other node, since a node could be in the middle of a synchronisation chain and on different interfaces there are different other nodes reachable which are also synchronizing the tangle. An example is shown in Figure \ref{fig:SynchronizationChain}.

%\begin{figure}
%    \centering
%    \includegraphics[width=0.27\textwidth]{Figures/SynchronizationChain.pdf}
%    \caption{Node 1 receives two head lists from node 2 and node 3. While setting up a synchronization chain, the node is aware to merge the two lists and forward it downstream to the other partners.}
%    \label{fig:SynchronizationChain}
%\end{figure}

%Thus, after the bootstrapping process, a node sends a special packet into the network to notify other nodes,
%that it is synchronizing the tangle. This packet is multicasted to all faces matching the packet with forwarding rule independent of how exact the match is. This way, the packet will travel all possible paths to find another synchronizing node. Since the heads have been requested once from this node, there is at least one upstream path. 
%As soon as another node is reached, which is also synchronising the Tangle, the node will reply with a special NDO confirming the route. The forwarding system will be monitoring these special NDO and extend the FIB, by adding an new FIB entry with the name of the synchronized data pointing towards the matching PIT entry. This way we ensure, bidirectional connectivity between the nodes.
%We mark each NDO with a nonce and a hop count. This way, we can understand duplicated routes and preferably use the shorter route. However, we keep all possible routes for fail-safety.

%In TCN, we are using a three way handshake, so the new created FIB entries will only be persistent, if the initializing node is sending another packet to confirm the new routes.  

%All forwarding entries created by TCN for the synchronization purpose are temporary and we use a heartbeat to reset the counter. This way, we can ensure, that the temporary FIB entries are removed if they are no longer reqired.

%The first multicast packet is an interest message named with the name of the data to be synchronized, a nonce and the postfix \texttt{findsyncpartner}: 
%\begin{verbatim}
%    <name>/<nonce>/findsyncpartner
%\end{verbatim}
%The special NDO that is replied is a has the same name and contains the hop count in the payload. 
%The last packet of the three way handshake is again an interest message with the postfix \texttt{heartbeat}. The same type of message will be also used for the heartbeat. 
%A heartbeat is answered with a NDO which also contains the hop count to be able to detect network changes. 
%Figure \ref{fig:HandshakeProcess} shows a flow diagram of the three way handshake.

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{Figures/HandshakeProcess.pdf}
    \caption{Scheme of the synchronization chain handshake procedure. First sending an interest to all matching FIB entries, next receiving a NDO to set time-limited forwarding rules, last completing the synchronization handshake and starting the heartbeat message procedure.}
    \label{fig:HandshakeProcess}
\end{figure}

After the synchronization routes are established successfully, the nodes can start to synchronize on the Tangle tips. In case a Tangle contains multiple tips received by a node, it has to merge the tips by eliminating duplicated entries in the list of tips.

In case a connection loss happened and the disconnected node extends the Tangle with new elements (e.g., the vehicle drives into a tunnel having no connection to the communication infrastructure), it will restart the bootstrapping of the Tangle after re-connecting to the network. Other synchronization partners will receive the changes and decide whether to accept or reject to the latest changes using acknowledgements.

%After establishing the required routes, the heads can be synchronised between the nodes. Thereby, it is important that the packets used by the synchronization protocol (pSync, ChronoSync, ...) are also forwarded to all matching %faces. This means, that a node may not only receive a single head list but multiple. 

%The merging of head lists is straight forward: It is only required to add up all element in the head list and eliminate the duplicated once. 

%While for synchronisation, it is obviously required that nodes are only, nodes can extend a tangle without having an connection. As soon as a node come back online, it restarts the bootstrapping. The other nodes will decide if they accept the changes by appending acknowledgements.

==> Tangle Centric Networking/tfn.tex <==
\section{Tangles Supporting Compute-Centric Architectures}
\label{sec:tfn}

The introduction of TCN have shown improvements via network level consensus and efficient management of data chunks (cf. Section~\ref{sec:evaluation}).
However, the concepts of Tangles are promising for compute-centric architectures as well.
For example, the \emph{electronic horizon} compute graph logic can be modeled using Tangles.
By doing so, the Tangle can be synchronized between execution nodes to coordinate the execution of computations across cloud and edge environments, and thus, ensure to fulfill application demands. 
Tangle Function Networking (TFN) is an extension of TCN supporting the coordination of computation state across multiple execution nodes in a distributed and transparent fashion.

%Tangle Function Networking (TFN) is an extension of TCN, where the compute graph of a function is expressed as tangle. In TFN the compute graph can be synchronized between nodes participating in the computation, which can help to perform better coordination and even to extend or modify already running computations. 
%We encode the compute graph in a tangle to be able to synchronize it using TCN. 
%This way, TFN supports cooperative computing, extensions of long running computation, a computation state and is more flexible than other in network computation systems such as NFN~\cite{sifalakis2014information} and NFaaS~\cite{krol2017nfaas}. 
%TFN is an application build on top of TCN, to demonstrate the full potential of synchronizing tangles. 

\subsection{Tangles as Compute Graphs}
TFN is aligned with the design principles of compute-centric architectures presented in Section~\ref{sec:background:ccn}.
A compute description (e.g., in NFN using the $\lambda$-calculus), or compute graph (as in CFN) is used by the architecture to resolve nodes in the network able to fulfill the compute request.
Compared to CRDTs used by CFN, we propose to use Tangles to model the compute graph for two reasons: (i) improve the resolution of execution nodes, and (ii) dynamic extension of the graph by other nodes during runtime.

A Tangle in TFN consists of two blocks: \emph{functions}, and \emph{data} (input, compute state or compute result). Each of these blocks are represented as individual elements in the Tangle (cf. Figure~\ref{fig:TFNComputeGraph}). 
For example, an element for a function call is used to instantiate a function and contains a pointer to the executable (byte code) of the function to be fetched by execution nodes if not already present.
Examples of a \emph{data} element representing a compute state can be the value of a variable in the compute stack or an intermediate results which dependent on computation state or the data to be synchronized across multiple execution nodes. 
Therefore, TFN supports stateful computations.
In case a compute result is available in the network, the Tangle is updated accordingly that subsequent consumer can quickly query the network for the result.

%\DENNIS{result verification is missing}

Furthermore, modelling a compute graph using Tangles allows for parallel processing of the entire graph, depending on the type of application.
In case multiple execution nodes are involved in the overall computation request, a node acknowledges the execution of a function and updates the Tangle accordingly (cf. Figure~\ref{fig:TFNComputeGraph}, \emph{computing-this}-note). 
This procedure allows to coordinate the execution of the entire compute graph across multiple execution nodes transparently and in a distributed fashion. For example, in case a node joins the overall computation process after a connection loss, it has to synchronize only the remaining parts of the overall computation graph to fulfill its contribution. Previous compute states, as labeled by acknowledgements in the Tangle, can be ignored.
Furthermore, it limits the probability that a function within the Tangle is executed in parallel by different nodes.

%TFN uses the same principle as NFN, function code is stored within NDOs an can be transported over the network. However, a request in TFN differs strongly: instead of encoding the computation workflow by using the $\lambda$-calculus, we use a tangle. The tangle represents the compute graph,
%it contains function calls, input data as well as the compute state. Each function call, input data, compute state and result is stored on an individual block of the tangle. Thereby, each block contains an identifier field, which describe the type.
%A function call block contains the name of the NDO storing the function code or the function code itself. A data block contains a name of a NDO storing input data and a compute state block contains a part of the current compute state or references to a NDO containing compute state.

%The compute state represents local variables (e.g stack variables) and intermediate results which depend on the process of the computation. Thus, TFN supports stateful computations.
%TODO. multiple functions access the same local variable., append local var as block. add it as parameter to multiple functions 
%To create a local variable, a block is append on the tangle pointing on the creator of the local variable. Not every local variable needs to be %appended, only those which should be synchronized. Next, a NDN-name is chosen for the local variable, and the name is used for any further function %that wants to operate on the variable. Whenever a function changes the state of the local variable it will add a new version and waits for %acknowledgement-blocks by the other nodes using the variable. The number of involved nodes is known by the compute graph (number of function call %blocks having the variable involved as parameter) and as soon as half of the nodes which took over and function call involving the variable sent added %their acknowledgement, the state is considered to be updated. 


%Results, intermediate results and local variables are appended as new (sub)-tangles on the function call they belong to. This way, for all participating nodes the current state of the computation is transparent.

%If one of the synchronizing nodes decides to compute a part of the compute graph, it will append a element to the tangle to tell other nodes this part of the computation is in execution (\emph{computing-this}-note). 
%This way an efficient multiprocessing is possible. 
%Depending on the requirements of the computation each individual part of a computation can be executed by multiple nodes, for example for mobile scenarios or to verify that results are correct. 

%Figure \ref{fig:TFNComputeGraph} shows an example for a compute graph. 

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/TFNComputeGraph.pdf}
    \caption{Compute Graph of the function call \texttt{func1(func2(data3),data1)} in TFN. This figure shows only logical compute graph excluding the second hash reference of the tangle.}
    \label{fig:TFNComputeGraph}
\end{figure}

%Any node who synchronizes this tangle can participate in the computation. Thereby, they only synchronize the blocks of the tangle which they require, which keeps the synchronization lightweight but efficient. This, when a node joins a computation it will only synchronizes the function call and input data as well as the latest compute state. Previous compute states are not required. 

\subsection{Compute Coordination Strategies}

While a Tangle in TFN allows to model coordination of the execution of functions, coordination strategies are required to decide which node computes which part of the overall computation.
To simplify TFN, we propose to use one of the existing solutions of existing compute-centric networks. 
For example, NFN provides several strategies according to the scenario (e.g., mobility~\cite{scherb2019execution}, or \cite{scherb2018smart} for long running computations), while CFN provides task scheduling to coordinate functions across worker nodes~\cite{krol2019compute}.
However, a Tangle can be used to model the compute flow of the overall computation as well. 
Compute nodes can already commit to execute a function using an acknowledgement and start to execute the function if the required data (e.g., intermediate result) is available in the network.

%To distribute computations in the network a strategy is required, to decide which node computes which part of the overall computation.
%Therefore, different approaches can be chosen. Here we will look into two cases: static and mobile scenarios. 
%In static scenarios forwarding and resolution strategies of NFN can be used~\cite{scherb2018smart,scherb2019execution}. The network decides based on load, data location etc where to compute a result. Thereby, the requesting node will send a message to the, asking to compute a result. Nodes holing parts of the input data or have fast access to the input data will synchronize the tangle and start executing parts of the computation. This is very similar to the 
%\emph{Find-Or-Execute}~\cite{scherb2018resolution} and the default forwarding strategy of NFN (\emph{To-Data-First}~\cite{sifalakis2014information}).
%By appending results to the tangle other nodes can take over and continue the computation. 

%In mobile and swarm scenarios, for example vehicular scenarios, a node can start a computation and other nodes in range can join computations by synchronizing the tangle. A tangle can be published by broadcasting the name in regular intervals and each node decides if it wants to participate. Every participating node can take over a part of the computation. Since, in mobile nodes may easily loose connections, each result should be computed by multiple nodes. How many nodes should compute each part of the computation is defined by a compute state, which is appended as block to the outermost computation. 

\subsection{Adding Computations to Compute Tangles}

The concept of Tangles allows extensions to the data structure during runtime. In TFN, this allows to modify the compute graph dynamically, e.g., to adapt to long running computations. 
For example in the \emph{electronic horizon} scenario (cf. Section~\ref{sec:use_cases}, to warn the driver about a hazardous situation on the junction ahead, nodes can append image processing computations of a camera deployed close to the junctions to the compute Tangle or append the processing result to the Tangle as additional input for the computation.
%Nodes can stop the execution of functions by appending intermediate results to the Tangle and extend the computation. 
Any node synchronizing the Tangle is able to verify the new element and accept or reject it. In case such element is accepted, everyone subsequent node benefits from the additional computation result which is produced. In case the element got rejected, the original Tangle remains in tact, and therefore, the applications using its compute result.

%\begin{itemize}
%    \item To overcome NFN restrictions of long workflow names, short name for workflow, rest in tangle, may be more efficient. 
%    \item ultra long running computation, make particular computations available and make it usable by others.
%    \item NFaaS already uses Manifest to describe computations, tangles can contribute here, e.g., to link to other functions or to get information of partial computations.
%    \item Does tangle also help stateful operations??
%\end{itemize}

==> Tangle Centric Networking/use_cases.tex <==
\section{Use Case Scenarios}
\label{sec:use_cases}

Distributed edge computing environments enable novel classes of application scenarios in different IoT domains. 
Examples include smart factories, healthcare systems, or connected and automated driving (e.g.,~\cite{Buyya:IoT:use_cases}).
In this paper, we consider a use case from the domain of connected and automated driving, based on the special characteristics of the scenario. 

\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{Figures/e_horizon_tcn.pdf}
    \caption{The \emph{electronic horizon} in a distributed edge environment. Data from different sources are collected and processed close to the origin, creating an environmental model used by automated driving logic.}
    \label{fig:electronic_horizon}
\end{figure}

\subsection{Automotive: Electronic Horizon for Highly Automated Driving}
\label{sec:use_cases:automotive}

It is evident that automated driving will rely on information from in-vehicle systems as well as data sources deployed outside the vehicle~\cite{Wang:2019}.
It is expected that driving logic in automated driving vehicles will take in several inputs ranging from built-in sensor data streams to context and external information (incl. road topology, localization, position of obstacles and moving objects, odometry, acceleration data, traffic volumes, etc.). 
The characteristics of such data are quite different in terms of volumes, popularity as well as validity, most of it generated at the edge of the communication infrastructure (cf.~\cite{Moustafa:rCDN:2017}).

Based on all information, an environmental model is created periodically -- e.g., the Local Dynamic Map (LDM)~\cite{Andreone:LDM:2010} -- serving as an input to the driving logic to further improve the driving quality.
Finally, the driving logic computes the output for steering the vehicle (steering angle, inputs to the gas \& brake pedals, switching signal lamps etc.)

On the road towards fully automated driving, the \emph{electronic horizon} describes a purely cloud-based virtual vehicle sensor using pre-defined data sources. 
These sources include map data, vehicle’s mobility model as well as additional data regarding the stretch of road ahead during a journey. 
As it is already available as a product for certain high class vehicle models (e.g., \cite{dSpace:EH:2010, Bosch:cHorizon:2020}), it forms a base line scenario for upcoming driving logic in automated driving vehicles.

Figure~\ref{fig:electronic_horizon} illustrates the electronic horizon in a distributed edge deployment. 
The fusion of all data and computation of the model require a high amount of computing power. 
Instead of sending all the data towards cloud backends, data can be collected, processed and augmented with other information by compute nodes on the delivery path close to its origin (cf.~\cite{grewe2017information}). 
Such approach is promising to reduce the massive amount of data to be transmitted towards cloud backends (see reverse CDN~\cite{Moustafa:rCDN:2017}), while increasing the overall quality of information for such scenario (e.g., enhance information from camera streams nearby).

\subsection{Challenges from the Use Case}

The presented use case introduces several challenges. 
The data to be collected is of different types (e.g., large vs. small volumes, popularity, etc.), while dynamically generated content from compute nodes challenges efficient dissemination.
From a communication and computing infrastructure perspective, data flows are reversing from downstream of cloud backends, towards upstream from devices close to the vehicle. The scenario challenges to \emph{understand} data points as well as to put data and computations into the right context (linking together) to be processed at the network edge.
From a vehicle perspective, the scenario challenges dynamically generated data and discovers the \emph{closest} compute node by taking the mobility aspect of the vehicle into account.


% for related work in which DLTs are used in shade of the use case:
% B-FICA and Block4Forensic a two proposals for a forensics blockchain for vehicle forensics and insurance


==> interactions.tex <==
\section{Interactions in TCN}

\subsection{Build-In Operations in TCN}
\label{sec:tangle:operations}

\DENNIS{STOPPED HERE}
\COMMENT{Here the sync part needs to go, we have that later in the sync section in detail}
\COMMENT{Move this behind the sync chapter}
\COMMENT{Push vs. Pull based communication in ICN - evtl. Ref to ''Mobile Data Repositories at the Edge''}

For updating the manifests, a synchronization mechanism such as PSync~\cite{Zhang:PSync:2017} or a similar synchronisation mechanism can be used. Another option is to use a
publish subscribe system where nodes holding the manifests (and so the content) subscribe to each others updates. 
By updating the manifests, the nodes see, if chunks were added to a NDO, were removed or updated. In case there were changes to chunks the node
holds, the node can update the chunks and a client will always receive the latest version. A scheme of synchronizing the MST and updating chunks between nodes is shown in Figure \ref{fig:TCNSyncExample}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/TCNSyncExample.pdf}
    \caption{Scheme of synchronizing the MST and updating chunks.}
    \label{fig:TCNSyncExample}
\end{figure}

Since the tangle representing the manifest document all changes on the chunks (and by that on the content), the network can provide functionality to
request any version of the file. A client can send the following requests to the network: 
\begin{itemize}
    \item \texttt{get(name)}: get the latest version of a NDO \\(also: \texttt{get\_latest(name)}).
    \item \texttt{get\_initial(name)}: get the initial version of a NDO.
    \item \texttt{get\_list(name)}: list all versions of a NDO.
    \item \texttt{get\_version(name, version)}: get a specific version of a NDO.
\end{itemize}

For all nodes which are synchronizing the manifest, further commands are available:
\begin{itemize}
    \item \texttt{update\_chunk(manifest\_name, chunk\_name, \\ new\_content)}: update a specific chunk in a specific manifest.
    \item \texttt{remove\_chunk(manifest\_name, chunk\_name)}: \\ remove a specific chunk from a manifest.
    \item \texttt{add\_chunk(manifest\_name, new\_chunk\_name, \\ chunk\_to\_append, new\_content)}: add a specific \\ chunk to a manifest. Append it to a specific existing chunk.
\end{itemize}

However, a command cannot be executed without the consensus of the other nodes. Whenever one of this operations is accepted, a new version
is created. This way, the file history is available to all nodes. This structure is comparable with block-chain data storage where in the block-chain only the hash value is stored, which references to the actual data. However, while a block-chain is a single decentralized data structure which is replicated by everyone, TCN brings 
one decentralized data structure per published content. Thus, the synchronization process of TCN is very lightweight compared to block-chain. Moreover, Tangles are more flexible then block-chain. They can be particularly synchronized and still be validated. More over, old stale information of the Tangle can also be dropped. 
This way, a publisher can decide to drop old versions of a file and don't need to 
continue storing all old version of a file, while nodes in the network can continue doing so. 



\DENNIS{MOVED TANGLE DESIGN UP IN CHAPTER}

\subsection{Logical Tangle Traversal}
Beside the cryptographical structure of a tangle, which is defined by which element is verified
by which other element, there is also a logical structure. The logical structure concerns the Structure
of the NDO and the chunks and is important for the node to handle requests and to perform operations on the Tangle.
The idea here is, that from the given tangle, a node creates a logical representation, so that it can easily traversal the tangle and serve requests like linear streaming or delivering a specific version of the entire NDO or of parts of it. For those kind of requests, the pure tangle structure is not sufficient, since it only allows traversing backwards. 
When a node starts synchronizing a tangle, it will store the blocks in the MST and beside it will keep create and store the logical representation for a fast reaction time.

To build the logical structure, a node will traverse the tangles from the head to the start. Thereby, it uses the property that the core elements have primary hash entries, which have a semantic meaning. Moreover, acknowledgements are not required for the logical structure of the NDO.

The goal is to create a graph that enables the node to easy traverse from the first to the last chunk in any available version of the NDO. 

Thus, the node will organize the blocks as following: Starting from the first block which references the first version of the first chunk a logical graph is created. Thereby a block points to its successor, extensions as well as to newer versions of itself. The pointers have a different type, so that when traversing the logical graph, it is easy to find elements one is looking for. 

For each version or extension of the content another pointer is added to the base version of the next block.
This way, it is fast to traverse the Tangle and to easily pick the different versions of the NDO or even of individual chunks. 

In general, this data structure is not required, since all information are stored in the tangle by using the primary hash pointer, but it is more efficient at run time to identify the relevant blocks. Figure \ref{fig:TangleLogicalStructure} shows the logical structure of a tangle as it would be used in TCN.


\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/TangleLogicalStructure.pdf}
    \caption{Logical Structure of the Tangle, which helps nodes to quickly find requested chunks}
    \label{fig:TangleLogicalStructure}
\end{figure}

%TODO, if we have space, we can talk here how getVersion etc is implemented

%TODO figures: elements and 





% TODO CHECK WHERE TO PUT THIS CONTENT??
%The manifest is stored in MST. Beside storing the manifest the MST is also synchronizing the manifests with the manifests of the same NDOs stored on different nodes. 
%In addition to improve the performance of the ICN forwarders for large NDO queries, the TCN architecture introduces a Manifest Synchronization Table (MST) as an additional data structure. 
%In the TCN forwarding plane, Tangles are stored in a dedicate MST data structure instead of being handled as a typical content object in the ICN forwarding plane (cf. Figure~\ref{fig:TCNArchitecture}).
%This has two reasons: (i) it allows to identify and operate on Tangles (e.g., synchronize its content due to updates), and (ii) avoids eviction of Tangles as potentially happen when handled in the ICN content store due to cache %management policies.

%\begin{figure}
%    \centering
%    \includegraphics[width=0.45\textwidth]{Figures/TCNArchitecture.pdf}
%    \caption{Scheme of the architecture of a TCN Node including the classic ICN/NDN forwarding pipeline.}
%    \label{fig:TCNArchitecture}
%\end{figure}

==> tfn.tex <==
\section{Tangles Supporting Compute-Centric Architectures}
\label{sec:tfn}

The introduction of TCN have shown improvements via network level consensus and efficient management of data chunks (cf. Section~\ref{sec:evaluation}).
However, the concepts of Tangles are promising for compute-centric architectures as well.
For example, the \emph{electronic horizon} compute graph logic can be modeled using Tangles.
By doing so, the Tangle can be synchronized between execution nodes to coordinate the execution of computations across cloud and edge environments, and thus, ensure to fulfill application demands. 
Tangle Function Networking (TFN) is an extension of TCN supporting the coordination of computation state across multiple execution nodes in a distributed and transparent fashion.

%Tangle Function Networking (TFN) is an extension of TCN, where the compute graph of a function is expressed as tangle. In TFN the compute graph can be synchronized between nodes participating in the computation, which can help to perform better coordination and even to extend or modify already running computations. 
%We encode the compute graph in a tangle to be able to synchronize it using TCN. 
%This way, TFN supports cooperative computing, extensions of long running computation, a computation state and is more flexible than other in network computation systems such as NFN~\cite{sifalakis2014information} and NFaaS~\cite{krol2017nfaas}. 
%TFN is an application build on top of TCN, to demonstrate the full potential of synchronizing tangles. 

\subsection{Tangles as Compute Graphs}
TFN is aligned with the design principles of compute-centric architectures presented in Section~\ref{sec:background:ccn}.
A compute description (e.g., in NFN using the $\lambda$-calculus), or compute graph (as in CFN) is used by the architecture to resolve nodes in the network able to fulfill the compute request.
Compared to CRDTs used by CFN, we propose to use Tangles to model the compute graph for two reasons: (i) improve the resolution of execution nodes, and (ii) dynamic extension of the graph by other nodes during runtime.

A Tangle in TFN consists of two blocks: \emph{functions}, and \emph{data} (input, compute state or compute result). Each of these blocks are represented as individual elements in the Tangle (cf. Figure~\ref{fig:TFNComputeGraph}). 
For example, an element for a function call is used to instantiate a function and contains a pointer to the executable (byte code) of the function to be fetched by execution nodes if not already present.
Examples of a \emph{data} element representing a compute state can be the value of a variable in the compute stack or an intermediate results which dependent on computation state or the data to be synchronized across multiple execution nodes. 
Therefore, TFN supports stateful computations.
In case a compute result is available in the network, the Tangle is updated accordingly that subsequent consumer can quickly query the network for the result.

%\DENNIS{result verification is missing}

Furthermore, modelling a compute graph using Tangles allows for parallel processing of the entire graph, depending on the type of application.
In case multiple execution nodes are involved in the overall computation request, a node acknowledges the execution of a function and updates the Tangle accordingly (cf. Figure~\ref{fig:TFNComputeGraph}, \emph{computing-this}-note). 
This procedure allows to coordinate the execution of the entire compute graph across multiple execution nodes transparently and in a distributed fashion. For example, in case a node joins the overall computation process after a connection loss, it has to synchronize only the remaining parts of the overall computation graph to fulfill its contribution. Previous compute states, as labeled by acknowledgements in the Tangle, can be ignored.
Furthermore, it limits the probability that a function within the Tangle is executed in parallel by different nodes.

%TFN uses the same principle as NFN, function code is stored within NDOs an can be transported over the network. However, a request in TFN differs strongly: instead of encoding the computation workflow by using the $\lambda$-calculus, we use a tangle. The tangle represents the compute graph,
%it contains function calls, input data as well as the compute state. Each function call, input data, compute state and result is stored on an individual block of the tangle. Thereby, each block contains an identifier field, which describe the type.
%A function call block contains the name of the NDO storing the function code or the function code itself. A data block contains a name of a NDO storing input data and a compute state block contains a part of the current compute state or references to a NDO containing compute state.

%The compute state represents local variables (e.g stack variables) and intermediate results which depend on the process of the computation. Thus, TFN supports stateful computations.
%TODO. multiple functions access the same local variable., append local var as block. add it as parameter to multiple functions 
%To create a local variable, a block is append on the tangle pointing on the creator of the local variable. Not every local variable needs to be %appended, only those which should be synchronized. Next, a NDN-name is chosen for the local variable, and the name is used for any further function %that wants to operate on the variable. Whenever a function changes the state of the local variable it will add a new version and waits for %acknowledgement-blocks by the other nodes using the variable. The number of involved nodes is known by the compute graph (number of function call %blocks having the variable involved as parameter) and as soon as half of the nodes which took over and function call involving the variable sent added %their acknowledgement, the state is considered to be updated. 


%Results, intermediate results and local variables are appended as new (sub)-tangles on the function call they belong to. This way, for all participating nodes the current state of the computation is transparent.

%If one of the synchronizing nodes decides to compute a part of the compute graph, it will append a element to the tangle to tell other nodes this part of the computation is in execution (\emph{computing-this}-note). 
%This way an efficient multiprocessing is possible. 
%Depending on the requirements of the computation each individual part of a computation can be executed by multiple nodes, for example for mobile scenarios or to verify that results are correct. 

%Figure \ref{fig:TFNComputeGraph} shows an example for a compute graph. 

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/TFNComputeGraph.pdf}
    \caption{Compute Graph of the function call \texttt{func1(func2(data3),data1)} in TFN. This figure shows only logical compute graph excluding the second hash reference of the tangle.}
    \label{fig:TFNComputeGraph}
\end{figure}

%Any node who synchronizes this tangle can participate in the computation. Thereby, they only synchronize the blocks of the tangle which they require, which keeps the synchronization lightweight but efficient. This, when a node joins a computation it will only synchronizes the function call and input data as well as the latest compute state. Previous compute states are not required. 

\subsection{Compute Coordination Strategies}

While a Tangle in TFN allows to model coordination of the execution of functions, coordination strategies are required to decide which node computes which part of the overall computation.
To simplify TFN, we propose to use one of the existing solutions of existing compute-centric networks. 
For example, NFN provides several strategies according to the scenario (e.g., mobility~\cite{scherb2019execution}, or \cite{scherb2018smart} for long running computations), while CFN provides task scheduling to coordinate functions across worker nodes~\cite{krol2019compute}.
However, a Tangle can be used to model the compute flow of the overall computation as well. 
Compute nodes can already commit to execute a function using an acknowledgement and start to execute the function if the required data (e.g., intermediate result) is available in the network.

%To distribute computations in the network a strategy is required, to decide which node computes which part of the overall computation.
%Therefore, different approaches can be chosen. Here we will look into two cases: static and mobile scenarios. 
%In static scenarios forwarding and resolution strategies of NFN can be used~\cite{scherb2018smart,scherb2019execution}. The network decides based on load, data location etc where to compute a result. Thereby, the requesting node will send a message to the, asking to compute a result. Nodes holing parts of the input data or have fast access to the input data will synchronize the tangle and start executing parts of the computation. This is very similar to the 
%\emph{Find-Or-Execute}~\cite{scherb2018resolution} and the default forwarding strategy of NFN (\emph{To-Data-First}~\cite{sifalakis2014information}).
%By appending results to the tangle other nodes can take over and continue the computation. 

%In mobile and swarm scenarios, for example vehicular scenarios, a node can start a computation and other nodes in range can join computations by synchronizing the tangle. A tangle can be published by broadcasting the name in regular intervals and each node decides if it wants to participate. Every participating node can take over a part of the computation. Since, in mobile nodes may easily loose connections, each result should be computed by multiple nodes. How many nodes should compute each part of the computation is defined by a compute state, which is appended as block to the outermost computation. 

\subsection{Adding Computations to Compute Tangles}

The concept of Tangles allows extensions to the data structure during runtime. In TFN, this allows to modify the compute graph dynamically, e.g., to adapt to long running computations. 
For example in the \emph{electronic horizon} scenario (cf. Section~\ref{sec:use_cases}, to warn the driver about a hazardous situation on the junction ahead, nodes can append image processing computations of a camera deployed close to the junctions to the compute Tangle or append the processing result to the Tangle as additional input for the computation.
%Nodes can stop the execution of functions by appending intermediate results to the Tangle and extend the computation. 
Any node synchronizing the Tangle is able to verify the new element and accept or reject it. In case such element is accepted, everyone subsequent node benefits from the additional computation result which is produced. In case the element got rejected, the original Tangle remains in tact, and therefore, the applications using its compute result.

%\begin{itemize}
%    \item To overcome NFN restrictions of long workflow names, short name for workflow, rest in tangle, may be more efficient. 
%    \item ultra long running computation, make particular computations available and make it usable by others.
%    \item NFaaS already uses Manifest to describe computations, tangles can contribute here, e.g., to link to other functions or to get information of partial computations.
%    \item Does tangle also help stateful operations??
%\end{itemize}
